Online (and Offline) Robust PCA: Novel Algorithms and Performance Guarantees

In this work, we study the online robust principal components' analysis (RPCA) problem. In recent work, RPCA has been defined as a problem of separating a low-rank matrix (true data), $L$, and a sparse matrix (outliers), $S$, from their sum, $M:=L + S$. A more general version of this problem is to recover $L$ and $S$ from $M:=L + S + W$ where $W$ is the matrix of unstructured small noise/corruptions. An important application where this problem occurs is in video analytics in trying to separate sparse foregrounds (e.g., moving objects) from slowly changing backgrounds. While there has been a large amount of recent work on solutions and guarantees for the batch RPCA problem, the online problem is largely open."Online" RPCA is the problem of doing the above on-the-fly with the extra assumptions that the initial subspace is accurately known and that the subspace from which $l_t$ is generated changes slowly over time. We develop and study a novel "online" RPCA algorithm based on the recently introduced Recursive Projected Compressive Sensing (ReProCS) framework. Our algorithm improves upon the original ReProCS algorithm and it also returns even more accurate offline estimates. The key contribution of this work is a correctness result (complete performance guarantee) for this algorithm under reasonably mild assumptions. By using extra assumptions -- accurate initial subspace knowledge, slow subspace change, and clustered eigenvalues -- we are able to remove one important limitation of batch RPCA results and two key limitations of a recent result for ReProCS for online RPCA. To our knowledge, this work is among the first few correctness results for online RPCA. Most earlier results were only partial results, i.e., they required an assumption on intermediate algorithm estimates.

==> aistats_main_arxiv.tex <==


\begin{abstract}
In this work, we study the online robust principal components' analysis (RPCA) problem. In recent work, RPCA has been defined as a problem of separating a low-rank matrix (true data), $\L:=[\ell_1, \ell_2, \dots \ell_{t}, \dots , \ell_{t_{\max}}]$, and a sparse matrix (outliers), $\S:=[x_1, x_2, \dots x_{t}, \dots, x_{t_{\max}}]$, from their sum, $\bm{M}:=\L + \S$. A more general version of this problem is to recover $\L$ and $\S$ from $\bm{M}:=\L + \S + \bm{W}$ where $\bm{W}$ is the matrix of unstructured small noise/corruptions. An important application where this problem occurs is in video analytics in trying to separate sparse foregrounds (e.g., moving objects) from slowly changing backgrounds. While there has been a large amount of recent work on solutions and guarantees for the batch RPCA problem, the online problem is largely open.``Online" RPCA is the problem of doing the above on-the-fly with the extra assumptions that the initial subspace is accurately known and that the subspace from which $\lt$ is generated changes slowly over time.

We develop and study a novel ``online" RPCA algorithm based on the recently introduced Recursive Projected Compressive Sensing (ReProCS) framework. Our algorithm improves upon the original ReProCS algorithm and it also returns even more accurate offline estimates. The key contribution of this work is a correctness result (complete performance guarantee) for this algorithm under reasonably mild assumptions. By using extra assumptions -- accurate initial subspace knowledge, slow subspace change, and clustered eigenvalues -- we are able to remove one important limitation of batch RPCA results and two key limitations of a recent result for ReProCS for online RPCA. To our knowledge, this work is among the first few correctness results for online RPCA. Most earlier results were only partial results, i.e., they required an assumption on intermediate algorithm estimates.%
%In this work we develop and study a novel online robust principal components' analysis (RPCA) algorithm based on the recently introduced ReProCS framework. Our algorithm significantly improves upon the original ReProCS algorithm and it also returns even more accurate offline estimates. The key contribution of this work is a correctness result for this algorithm under relatively mild assumptions. By using extra (but usually valid) assumptions we are able to remove one important limitation of batch RPCA results and two important limitations of a recent result for ReProCS for online RPCA. To the best of our knowledge, this work is among the first correctness results for online RPCA. %-- accurate initial subspace knowledge, slow subspace change, and clustered stable eigenvalues --
\end{abstract}

\section{Introduction}
Principal Components Analysis (PCA) is a tool that is frequently used for dimension reduction. Given a matrix of data, PCA computes a small number of orthogonal directions that contain most of the variability of the data. PCA for relatively noise-free data is easily accomplished via singular value decomposition (SVD). %of $\D$. % and retaining the singular vectors corresponding to the largest singular values.
The robust PCA (RPCA) problem, which is the problem of PCA in the presence of outliers, is much harder. In recent work, Cand\`{e}s et al. \cite{rpca} posed it as a problem of separating a low-rank matrix, $\L$, (true data) and a sparse matrix, $\S$, (outliers\footnote{Since an outlier is something that occurs occasionally, it is well modeled using a sparse matrix of corruptions.}) from their sum, $\bm{M}:=\L+\S$. They proposed a convex program called principal components' pursuit (PCP) that provided a provably correct batch solution to this problem under mild assumptions. The same program was also analyzed in Chandrasekharan et al. \cite{rpca2} and later in Hsu et al. \cite{rpca_zhang}. Since these works, there has been a large amount of work on batch RPCA methods and performance guarantees. The more general case, $\bm{M}:=\L + \S + \bm{W}$ where $\bm{W}$ is unstructured small noise/corruptions, has also been studied in later works, e.g., \cite{stablePCP}.

When RPCA needs to be solved in a recursive fashion for sequentially arriving data vectors it is referred to as incremental or recursive or dynamic or ``online" RPCA. %By online or recursive we mean obtain estimates of the sparse matrix columns and of the low-rank matrix columns and its subspace using the previous estimates, rather than re-solving the entire problem at each time $t$. , or an initial estimate of the low-dimensional subspace, ``Online dynamic RPCA" may be a better term to describe this problem.
``Online" RPCA assumes that (i) a short sequence of outlier-free (sparse component free) data vectors is available or that there is another way to get an estimate of the initial subspace of the true data (without outliers); and that (ii) the subspace from which $\lt$ is generated is either fixed or changes slowly over time. We put ``online" in quotes here to stress that the ``online" problem formulation uses extra assumptions beyond what are used by batch RPCA.
An important application where the RPCA problem occurs is one of separating a video sequence into foreground and background layers \cite{rpca}. Video layering is a key first step to simplifying many video analytics and computer vision tasks, e.g., video surveillance (to track moving foreground objects), background video recovery and subspace tracking in the presence of frequent foreground occlusions or low-bandwidth mobile video chats or video conferencing (can transmit only the foreground layer).
%Video layering is an important first step for automatic video surveillance and many other streaming video analytics tasks.
In videos, the foreground typically consists of one or more moving persons or objects and hence is a sparse image. The background images (in a static camera video) usually change only gradually over time, e.g., moving lake waters or moving trees in a forest, and the changes are global \cite{rpca}. Hence they are well modeled as being dense and lying in a low-dimensional subspace that is fixed or slowly changing. We show an example in Fig. \ref{expt}. In many videos, it is also valid to assume that a short initial sequence is available without any foreground objects, i.e., (i) holds.
Other RPCA applications include recommendation system design, survey data analysis \cite{rpca}, anomaly detection in dynamic social (or computer) networks \cite{mateos_anomaly} or dynamic magnetic resonance imaging (MRI) based region-of-interest tracking \cite{candes_mri}. In many of these, an online solution is desirable.%
%, e.g., moving lake waters or moving trees in a forest. Also, the changes are global (dense) \cite{rpca}. %In most video applications, it is valid to assume that an initial short sequence of background-only frames is available and this can be used to estimate the initial subspace via SVD.,
%In case of a static camera video,
%Video layering is a key first step to simplifying many video analytics and computer vision tasks, e.g., video surveillance (to track moving foreground objects), background video recovery and subspace tracking in the presence of frequent foreground occlusions or low-bandwidth mobile video chats or video conferencing (can transmit only the foreground layer).


%??? add figure from mod-PCP paper - Fig 6c and lake with large object??.
%\input{CurtainFigure}

\subsection{Problem Definition} \label{probdef}
At time $t$ we observe a data vector $\mt \in \R^n$ that satisfies
\bea
\mt = \lt + \xt + \wt, \ \text{for} \  t = t_{\train}+1, t_{\train}+2, \dots, t_{\max}.
\label{orpca_eq}
\eea
%for $t = t_{\train}+1, t_{\train}+2, \dots, t_{\max}$.
For $t=1,2,\dots, t_\train$, $\xt=0$, i.e., $\mt = \lt + \wt$.
%with the possibility that $t_{\max}$ can be infinity too.
Here  $\lt$ is a vector that lies in a low-dimensional subspace that is fixed or slowly changing in such a way that the matrix $\bm{L}_t:=[\l_1, \l_2, \dots, \lt]$ is a low-rank matrix for all but very small values of $t$; $\xt$  is a sparse (outlier) vector; and $\wt$ is small modeling error or noise. We use $\T_t$ to denote the support set of $\xt$ and we use $\P_t$ to denote a basis matrix for the subspace from which $\lt$ is generated.
For $t > t_\train$, the goal of online RPCA is to recursively estimate $\lt$ and its subspace $\Span(\P_t)$,  and $\xt$ and its support, $\T_t$, as soon as a new data vector $\mt$ arrives or within a short delay\footnote{By definition, a subspace of dimension $r>1$ cannot be estimated immediately since it needs at least $r$ data points to estimate}.
Sometimes, e.g., in video analytics, it is often also desirable to get an improved offline estimate of $\xt$ and $\lt$ when possible. %In these cases, one can go backwards in time and get much more accurate final estimates of $\xt$ and $\lt$ after an accurate enough estimate of the new subspace is obtained.
We show that this is an easy by-product of our solution approach.


The initial $t_\train$ outlier-free measurements are used to get an accurate estimate of the initial subspace via PCA. For video, this assumption corresponds to having a short initial sequence of background-only images, which can often be obtained.
%The sparse vector $\xt$ and its support $\T_t$ and the vector $\lt$ can be recovered as soon as a new $\mt$ arrives. But an $r$-dimensional subspace needs $r$ linearly independent vectors generated from it to completely specify it; if only erroneous versions of the vectors are available, then many more are needed. Thus, the subspace of $\lt$ can only be estimated after a delay.
%the subspace, by definition, cannot be estimated immediately (an $r$-dimensional subspace is defined by $r$ linearly independent vectors, when the data has errors we need more than $r$ vectors to get a good estimate).
%
%In our older work on this topic \cite{rrpcp_icassp15,rrpcp_isit15}, we actually overestimated the subspace from which $\lt$ was generated. We were actually estimating the subspace spanned by $\l_1, \l_2, \dots \lt$ at time $t$ and this was being done by only adding directions to the previous subspace estimate without deleting any. In this work we remove this limitation by also introducing an automatic algorithm to delete old directions. Moreover, in older work, we assumed that the $\lt$'s are mutually independent over time. In this work we also state a result which replaces this assumption by a more practical autoregressive model on the $\lt$'s.
%

In many applications, it is actually the sparse outlier $\xt$ that is the quantity of interest. The above problem can thus also be interpreted as one of {\em online sparse matrix recovery in large but structured noise $\lt$ and unstructured small noise $\wt$}.
%
% (i.e. it does not satisfy condition \ref{xmin_cond}) is not sparse enough or when all its nonzero entries
The unstructured noise, $\wt$, often models the modeling error. For example, when some of the corruptions/outliers are small enough to not significantly increase the subspace recovery error, these can be included into $\wt$ rather than $\xt$.
%not large enough (to be detectable by the proposed algorithm), these can be included into $\wt$. Or, more generally, $\xt$ may also be not be exactly sparse and then again the small entries of $\xt$ will form $\wt$. (nonzero entries of $\xt$)
Another example is when the $\lt$'s form an approximately low-rank matrix.% In this case, we can compute the left singular vectors corresponding to the top $r$ singular values of $\bm{L}_t$, and we can let $\wt$ be replaced by the projection of $\lt$ into the space perpendicular to that spanned by these top $r$ singular vectors. % (compared to the energy along the changed subspace)
%a similar thing happens with the $\lt$'s:

\begin{figure}[t!]%{0.8\textwidth}
\centering
%\includegraphics[width=\linewidth]{figures/lake_view.eps} foreground-background difference on foreground support ($\xhatt$)
\includegraphics[width=\linewidth]{Figures/lake_view.eps} \vspace{-0.9in}
\caption{\small{The first column shows the video of a moving rectangular object against moving lake waters' background. The object and its motion are simulated while the background is real. In the next two columns, we show the recovered background ($\lhatt$) and the recovered foreground support ($\That_t$) using  Automatic ReProCS-cPCA (labeled ReProCS in the figure). The algorithm parameters are set differently for the experiments (see Sec. \ref{expts}) than in our theoretical result. Notice that the foreground support is recovered mostly correctly with only a few extra pixels and the background appears correct too (does not contain the moving block). The quantitative comparison is shown later in Fig. \ref{sims}.
The next few columns show background and foreground-support recovery using some of the existing methods discussed in Sec. \ref{relwork}.}}
\label{lake_view} \label{expt}
\end{figure}

\subsection{Related Work} \label{relwork}
%Some other work that also studies the online MC problem (defined differently from above) includes \cite{sequentialSVD,grouse,petrels,local_conv_grouse}. We discuss the connection with the idea from \cite{sequentialSVD} in Sec \ref{algos}. The algorithm from \cite{grouse}, grouse, is a first order stochastic gradient method. A  result for its local convergence is obtained in \cite{local_conv_grouse}. The algorithm of \cite{petrels}, petrels, is a second order stochastic gradient method. It is shown in \cite{petrels} that it converges to the stationary point of  the cost function it optimizes. The advantage of petrels and grouse is that they do not need initial subspace knowledge.% Our algorithms could also benefit from using their approach for initialization. %For our approach proposed above, when the initial subspace knowledge is not available or initial complete data is not available, we can also use the PETRELS or GROUSE ideas for initialization.  The result depended on intermediate algorithm estimates.
%%
%%Grassmanian Rank-One Update Subspace Estimation (GROUSE) \cite{grouse} and  Parallel Subspace Estimation and Tracking by Recursive Least Squares From Partial Observations (PETRELS) \cite{petrels}.
%and hence was not a correctness result A piecewise batch RPCA approach called modified-PCP was introduced and analyzed in \cite{zhan_pcp_jp}.
Solutions for online RPCA have been analyzed in recent works  \cite{rrpcp_perf}, \cite{xu_nips2013_1}, \cite{rrpcp_icassp15,rrpcp_isit15}. The work of \cite{rrpcp_perf} introduced the Recursive Projected Compressive Sensing (ReProCS) algorithmic framework and obtained a partial result for it. Another approach for online RPCA (defined differently from above) and a partial result for it were provided in \cite{xu_nips2013_1}. We use the term {\em partial result} to refer to a performance guarantee that depends on intermediate algorithm estimates satisfying certain properties. We will see examples of this in Sec. \ref{discussion} when we discuss the above results.
In very recent work \cite{rrpcp_icassp15,rrpcp_isit15}, a {\em correctness result} for ReProCS was obtained. The term {\em correctness result} refers to a complete performance guarantee, i.e., a  guarantee that only puts assumptions on the input data (here $\mt$) and/or on the algorithm initialization, but not on intermediate algorithm estimates.%

Other somewhat related work includes \cite{xu_nips2013_2} (online PCA with contaminated data that is not modeled as being sparse) and \cite{zhan_pcp_jp} (modified-PCP, a piecewise batch method). All the above results are discussed Sec. \ref{discussion}.

Some other works, such as \cite{grass_undersampled}(GRASTA), \cite{sequentialSVD} (adaptive-iSVD), \cite{Li03anintegrated} (incremental Robust Subspace Learning) or \cite{xu2013gosus} (GOSUS), \cite{mateos_anomaly,mateos_anomaly2}, \cite{chouvardas2015robust}, \cite{songimage}, \cite{vinjamuri2015sparse}
only provide an online RPCA algorithm without guarantees. We do not discuss these here. As demonstrated by the experimental comparisons shown in \cite{rrpcp_tsp} and in
\cite[Fig 6]{zhan_pcp_jp}, when the outlier support is large and changes in a correlated fashion over time, ReProCS-based algorithms significantly outperform most of these, besides also outperforming batch methods such as PCP and robust subspace learning (RSL) \cite{rpca,Torre03aframework}. This is also evident from Fig. \ref{expt} and Fig. \ref{sims}.
%For experiments comparing the ReProCS algorithm from this paper with these methods, please see Fig. \ref{expt} and Fig. \ref{sims}.
%It is shown to be better than adaptive-iSVD \cite{sequentialSVD}, iRSL \cite{Li03anintegrated}, GRASTA \cite{grass_undersampled}, GOSUS \cite{xu2013gosus},  PCP \cite{rpca,alm}, RSL \cite{rpca,Torre03aframework}, modified-PCP \cite{zhan_pcp_jp}.
%A somewhat related work is \cite{xu_nips2013_2}. The algorithm and result in this work are for online PCA in contaminated data with ``contamination" being anything that is ``far" from the data subspace. This does not model the outlier as a sparse vector but defines anything that is far from the data subspace as an outlier
%

%We explain below how the current work significantly improves upon this result.
%As shown in \cite{rrpcp_tsp} and in \cite[Fig 6]{zhan_pcp_jp}, for both simulated data and real video sequences, when the outlier support changes are correlated over time and/or when background changes significantly over time, ReProCS is significantly better than many other recursive adaptive-iSVD\cite{sequentialSVD}, iRSL \cite{Li03anintegrated}, GRASTA \cite{grass_undersampled}, GOSUS \cite{xu2013gosus}), batch (PCP \cite{rpca,alm}, RSL \cite{rpca,Torre03aframework}) and piecewise batch (modified-PCP \cite{zhan_pcp_jp}) methods for RPCA.%(1) The current algorithm and its correctness result allow for both small corruptions and large outliers. We also show that a simple by-product of our algorithm is offline recovery of $\xt$ and $\lt$ that is much more accurate than the online one.

\subsection{Contributions}
%In this work we develop and study {\em Automatic ReProCS-cPCA} which is a significantly improved algorithm compared to the original one \cite{rrpcp_perf,rrpcp_icassp15}.
In this work we develop and study an algorithm based on the ReProCS idea introduced and studied in \cite{rrpcp_perf,rrpcp_icassp15,rrpcp_isit15}. We call it Automatic ReProCS with cluster PCA (ReProCS-cPCA). This is an improved ReProCS algorithm compared to the ones studied in previous work. (1) It is able to automatically detect subspace changes within a short delay; is able to correctly estimate the number of directions added or deleted; and is also able to correctly estimate the clusters of eigenvalues along the existing directions. This is important because it is impractical to assume that a subspace change time or the exact number of added or removed directions is known. Additionally, these estimates themselves are relevant for applications such as understanding dynamic social networks' structural changes in the presence of outliers. While many heuristics exist to detect sudden subspace changes, we provide an approach for correctly detecting slow subspace changes within a short delay. (2) Moreover it is able to accurately estimate both the newly added subspace as well as the newly deleted subspace. The latter is done by re-estimating the current subspace using an approach called cluster PCA (cPCA). The basic cPCA idea was introduced in \cite{rrpcp_perf}. The current work uses that idea to develop an automatic algorithm. The cPCA step ensures that the estimated subspace dimension does not keep increasing with time. (3) The current algorithm also returns more accurate offline estimates.
The algorithms studied in \cite{rrpcp_perf,rrpcp_icassp15} could not do (1) and (3). The algorithms studied in \cite{rrpcp_icassp15,rrpcp_isit15} did not do (2) and (3).

%The power of a slightly modified ReProCS algorithm based on the above ideas is shown in Fig. \ref{expt}.

The {\em main} contribution of this work is a correctness result (complete performance guarantee) for the proposed algorithm under relatively mild assumptions on $\lt$, $\xt$, and $\wt$. To our knowledge, this and \cite{rrpcp_icassp15,rrpcp_isit15} are the first correctness results for online RPCA. The result obtained here removes two key limitations of \cite{rrpcp_icassp15,rrpcp_isit15}. (1) First, we obtain a result for the case where the $\lt$'s can be correlated over time (follow an autoregressive (AR) model) where as the result of \cite{rrpcp_icassp15,rrpcp_isit15} needed mutual independence of the $\lt$'s. This models mostly static backgrounds in which changes are only due to independent variations at each time, e.g., light flickers. However, a large class of background image sequences change due to factors that are correlated over time, e.g., moving waters. This can be better modeled using an AR model.
(2) Second, with one extra assumption -- that the eigenvalues of the covariance matrix of $\lt$ are clustered for a period of time after the previous subspace change has stabilized -- we are able to remove another significant limitation of \cite{rrpcp_icassp15,rrpcp_isit15}. That result needed the rank of $\L$ to grow as $\bigo(\log n)$ while our result allows it to grow as $\bigo(n)$. Batch methods such as PCP allow the rank to grow almost linearly with $n$. The clustered eigenvalues assumption is valid for data that has variability at different scales - large scale variations would result in the first (largest eigenvalues') cluster and the smaller scale variations would form the later clusters.
%The reason for this significant relaxation is that, for ReProCS-cPCA, the dimension of the estimated subspace {\em does not} keep growing with time.

Because we use extra assumptions -- accurate initial subspace knowledge, slow subspace change, and clustered eigenvalues -- we are able to remove an important limitation of batch methods \cite{rpca,rpca2,rpca_zhang}. As we explain in Sec. \ref{discussion}, our result requires an order-wise looser bound on the number of time instants for which a particular index $i$ can be outlier-corrupted compared to these results. In other words, it allows significantly more correlated changes of the outlier support over time. This is important in practice, e.g., in video, foreground objects do not randomly jump around; in social networks, once an anomalous pattern starts to occur, it remains on many of the same edges for a while. The clustered eigenvalues assumption is discussed above. Accurate initial subspace knowledge and slow subspace change were discussed earlier (just above Sec. \ref{probdef}).
%We discuss the above points in detail in Sec. \ref{discussion}.% (but usually valid)

The novelty in the proof techniques used in this work is summarized in Sec. \ref{novelty}. The proof relies on the $\sin \theta$ theorem \cite{davis_kahan} (that bounds the effect of a perturbation on a Hermitian matrix's top eigenvectors) and the matrix Azuma inequality \cite{tail_bound}.

%relevant for many applications This extra assumption is needed to analyze the cluster PCA step that is used to delete the old directions from the subspace estimate.
% foreground objects are often slow moving or also occasionally static for short periods of time
%, e.g., in video foreground objects do not randomly jump around. In other applications too, when outliers appear, they remain for a while in roughly the same region.
%we allow this number to be a constant fraction of the total number of time instants, while PCP either requires this number to be $1/r$ times a constant fraction or requires this set to be uniformly random. Here $r$ is the rank of the matrix $\bm{L}_t$.

%We show that a simple by-product of our algorithm is offline recovery of $\xt$ and $\lt$ that is much more accurate than the online one. Another byproduct is a method for slow subspace change detection in the presence of outliers. This is relevant for applications such as understanding the (slow) structural changes to the connectivity patterns of dynamic social networks in the presence of outliers. While many approaches exist to detect sudden subspace change, we provide an approach for reliably detecting slow subspace changes.


%Our result uses the overall proof approach introduced in \cite{rrpcp_perf} that provided a partial result for online RPCA. The most important new insight needed to get a complete result is described in Sec \ref{algos}. %New proof techniques are needed for this line of work because almost all existing works only analyze batch algorithms that solve a different problem. Also, as explained in Sec \ref{algos}, the standard PCA procedure cannot be used in the subspace update step and hence results for it also not applicable.



\subsection{Notation}
%Notice that for a

%?? add more

We use the interval notation $[a, b]$ to mean all of the integers between $a$ and $b$, inclusive, and similarly for $[a,b)$ etc.
 For a set $\mathcal{T}$, $|\mathcal{T}|$ denotes its cardinality and $\bar{\mathcal{T}}$ denotes its complement set. We use $\emptyset$ to denote the empty set.

We use $'$ to denote a vector or matrix transpose.
The  $l_p$-norm of a vector and the induced $l_p$-norm of a matrix are denoted by $\| \cdot \|_p$.
For a vector $\bm{x}$ and set $\T$, $\bm{x}_{\mathcal{T}}$ is a smaller vector containing the entries of $\bm{x}$ indexed by entries in $\mathcal{T}$.
We use $\I$ to denote the identity matrix.
Define $\I_{\mathcal{T}}$ to be an $n \times |\mathcal{T}|$ matrix of those columns of the identity matrix indexed by entries in $\mathcal{T}$. For a matrix $\bm{A}$, define $\bm{A}_{\mathcal{T}} := \bm{AI}_{\mathcal{T}}$.
%
For matrices $\bm{P}$, $\bm{Q}$ where the columns of $\bm{Q}$ are a subset of the columns of $\bm{P}$, $\bm{P} \setminus \bm{Q}$ refers to the matrix of columns in $\bm{P}$ and not in $\bm{Q}$.
For a matrix $\bm{H}$, $\bm{H}\overset{\mathrm{EVD}}= \bm{U\Lambda U}'$ denotes its reduced eigenvalue decomposition.
For Hermitian matrices $\bm{A}$ and $\bm{B}$, the notation $\bm{A}\preceq\bm{B}$ means that $\bm{B}-\bm{A}$ is positive semi-definite. %V' denotes its singular value decomposition.

For a matrix $\bm{A}$, the restricted isometry constant (RIC) $\delta_s(\bm{A})$ is the smallest real number $\delta_s$ such that
\[
(1-\delta_s)\|\bm{x}\|_2^2 \leq \|\bm{Ax}\|_2^2 \leq (1+\delta_s) \|\bm{x}\|_2^2
\]
for all $s$-sparse vectors $\bm{x}$ \cite{candes_rip}.  A vector $\bm{x}$ is $s$-sparse if it has $s$ or fewer non-zero entries.

We refer to a matrix with orthonormal columns as a {\em basis matrix}. Thus, for a basis matrix $\bm{P}$, $\bm{P}'\bm{P} = \bm{I}$.
For basis matrices $\Phat$ and $\P$, $\mathrm{dif}(\Phat,\P):= \|(\I - \Phat \Phat') \P \|_2$ quantifies error between their range spaces.%

\subsection{Paper organization}
This paper is organized as follows. We discuss the data models and the main results for the proposed algorithm in Sec. \ref{models}. The Automatic ReProCS-cPCA algorithm is developed in Sec. \ref{algo_sec}. The stepwise algorithm is summarized in Algorithm \ref{reprocsdet}. The proof outline of our main result is given in Sec. \ref{outline}. This section also helps understand the algorithm better and explains the novelty in the proof techniques. The lemmas for proving the main result, the proof of the main result and the proofs of the main lemmas are given in Sec. \ref{pf_thm1_cor}. The key lemmas needed to prove the main lemmas are proved in Sec. \ref{3_pfs} (lemmas for analyzing the projection-PCA based subspace addition step) and in Sec. \ref{3_pfs_del} (lemmas for analyzing the cluster PCA based subspace deletion step). These are the long sections that contain the new proofs that rely on the matrix Azuma inequality \cite{tail_bound}. This is needed because the $\lt$'s are now correlated over time. Simulation experiments comparing the proposed algorithm to some existing batch and online RPCA algorithms are described in Sec. \ref{expts}. Conclusions are given in Sec. \ref{conclude}.% (or in the Appendix in case the lemma is similar to a lemma from past work)


\section{Data models and main results} \label{models}
%\label{Problem Definition and Assumptions}
In this section, we give the data models and correctness results for our proposed algorithm, Automatic ReProCS-cPCA, and for its simplification, Automatic ReProCS. The algorithm itself is developed in Sec \ref{algo_sec} and the complete stepwise algorithm is summarized in Algorithm \ref{reprocsdet}. We give below the model on the outlier support sets $\T_t$,  the model on $\lt$, and the denseness assumption. Using these, we state the result for Automatic ReProCS in Sec. \ref{noclust_result}. In Sec. \ref{clust_result}, we state the clustering assumption and give the correctness result for Automatic ReProCS-cPCA. The results are discussed in Sec. \ref{discussion}.


%where we also explain why it works. The complete stepwise algorithm is listed in Algorithm \ref{reprocsdet}. We begin by giving the model on the outlier support set, $\T_t$. Next, in Sec \ref{indep_lt}, we state the assumptions on $\lt$ and the correctness result for the case when the $\lt$'s are assumed to be mutually independent over time. Finally in Sec \ref{correl_lt}, we state the most general form of the result that allows the $\lt$'s to follow an autoregressive (AR) model. In later sections, we only prove the correlated case result and the independent case one follows as its corollary.
%By stating the results, this way, the other assumptions on $\lt$ are easier to follow
% (Auto-On/Off-Add-Del-ReP)

\subsection{Model on the outlier support set, $\T_t$} %given in Model \ref{general_model}. Both this model and its generalization are the same as those introduced in \cite{rrpcp_icassp15,rrpcp_isit15}
We give here one simple and practically relevant special case of the most general assumptions (Model \ref{general_model}) on the outlier support sets $\T_t$. It requires that the $\T_t$'s have {\em some} changes over time and have size less than $s$. An example of this is a video application consisting of a foreground with a 1D object of length $s$ or less that remains static for at most $\beta$ frames at a time. When it moves, it moves {\em downwards (or upwards, but always in one direction)} by at least $\frac{s}{\rrho}$ pixels, and at most $\frac{s}{\rho_2}$ pixels. Once it reaches the bottom of the scene, it disappears. The maximum motion is such that, if the object were to move at each frame, it still does not go from the top to the bottom of the scene in a time interval of length $\alpha$. This is ensured if $\frac{s}{\rho_2} \alpha \le n$. Anytime after it has disappeared another object could appear. A visual depiction of this model is shown in Fig. \ref{supportfig}.
%We have used this example only to explain the idea. Instead, one could also have multiple objects moving in arbitrary directions as long as given in the supplementary material). %Also see Fig. \ref{supportfig}.
We have used this ``one object moving in one direction" example  to only explain the idea in a simple fashion. Instead, one could also have multiple moving objects and arbitrary motions, as long as the union of their supports follows the assumptions of Model \ref{sbyrho} below or those given later in Model \ref{general_model}. These models were introduced in \cite{rrpcp_isit15}.

\begin{sigmodel}[model on $\T_t$]\label{sbyrho}
Let $t^k$, with $t^k < t^{k+1}$, denote the times at which $\T_t$ changes and let $ \T^{[k]}$ denote the distinct sets.
For an integer $\alpha$, %(we set its value in Theorem \ref{thm1}), assume the following.
\ben
\item assume that $\T_t = \T^{[k]}$ for all times $t \in [t^k, t^{k+1})$ with $(t^{k+1} - t^k) < \beta$ and $|\T^{[k]}| \le s$;
\item let $\rrho$ be a positive integer so that for any $k$,
$
\T^{[k]} \cap \T^{[k+\rrho ]} = \emptyset;
$
assume that
$
{\rrho}^2 \beta \leq  0.0001 \alpha;
$

\item for any $k$,
$
\sum_{i=k+1}^{k+\alpha} \left|\T^{[i]} \setminus \T^{[i+1]}\right| \le n
$ and for any $k < i \le k+\alpha$,
$
(\T^{[k]} \setminus \T^{[k+1]}) \cap (\T^{[i]} \setminus \T^{[i+1]}) = \emptyset
$
(one way to ensure the first condition is to require that for all $i$, $|\T^{[i]} \setminus \T^{[i+1]}| \le \frac{s}{\rho_2}$ with $\frac{s}{\rho_2}\alpha \le n$).
%(One way to ensure $\sum_{i=k+1}^{k+\alpha}|\T^{[i]} \setminus \T^{[i+1]}| \le n$ is to require that  for all $i$, $|\T^{[i]} \setminus \T^{[i+1]}| \le \frac{s}{\rho_2}$ with $\frac{s}{\rho_2}\alpha \le n$.)
\een
In this model, $k$ takes values $1,2, \dots $; the largest value it can take is $t_{\max}$. We set $\alpha$ in the Theorem.
% (this will happen if $\T_t$ changes at every time).
\end{sigmodel}
%We note that the above is a simple special case of the most general model that works for our result.
%The video moving object example satisfies the above model as long as $\rho^2 \beta \le 0.0001 \alpha$. This becomes clearer from Fig. \ref{supportfig}.

\begin{figure}[t]
%\includegraphics[height=5cm, width=3.5cm]{Figures/Support_Change_1.pdf}
\centering
\begin{subfigure}{.5\linewidth}
\centering
\includegraphics[height=5cm, width=3.5cm]{Figures/Support_Change_1.pdf}
\caption{$\rho=3$ and $\beta=5$ case}
\end{subfigure}
\begin{subfigure}{.3\linewidth}
\centering
\includegraphics[height=5cm, width=2cm]{Figures/Support_Change_Disjoint.pdf}
\caption{$\rho=1$ and $\beta=1$ case}
\end{subfigure}
%\vspace{-0.15in}
\caption{\small{Examples of Model \ref{sbyrho}. (a) shows a 1D object of length $s$ that moves by at least $s/3$ pixels at least once every $5$ frames (i.e., $\rho=3$ and $\beta=5$). (b) shows the object moving by $s$ pixels at every frame  (i.e., $\rho=1$ and $\beta=1$). (b) is an example of the best case for our result - the case with the smallest $\rho,\beta$ ($\T_t$'s  mutually disjoint)
}}
\vspace{-0.1in}
\label{supportfig}
\end{figure}


%Often a Gaussian assumption is also used again primarily for simplicity of analysis (even though in practice most sensor data or noise is bounded). For example in the video case, the background images are always slowly changing but the subspace in which they lie may actually change with time rather than being fixed.
%Of course since things don't change abruptly, one would also assume that $\Sigma_t$ is ``slowly changing".   $\Sigma_t =  \P_t \Lamt \P_t'$ where

%\subsection{Models on $\ell_t$ and main result -- mutually independent $\ell_t$'s case}  that changes slowly with time

\subsection{Model on $\ell_t$}
A common model for data that lies in a low-dimensional subspace is to assume that, at all times, it is independent and identically distributed (iid) Gaussian with zero mean and a fixed {\em low-rank} covariance matrix $\bm\Sigma$. However this can be restrictive since, in many applications, data statistics change with time, albeit slowly. To model this perfectly, one would need to assume that $\lt$ is zero mean with covariance matrix $\bm{\Sigma}_t$ at time $t$. If $\bm{\Sigma}_t \overset{\mathrm{EVD}}{=} \P_t \Lamt \P_t'$, this means that both $\P_t$ and $\Lamt$ can change at each time $t$, though slowly. This is the most general model but it has an identifiability problem if the goal is to estimate the subspace from which $\lt$ was generated, $\Span(\P_t)$.
The subspace cannot be estimated with one data point. If it is $r$-dimensional, it needs at least $r$ data points. So, if $\P_t$ changes at each time, it is not clear how one can estimate all the subspaces. To resolve this issue, a general enough but tractable option is to assume that $\P_t$ is piecewise constant with time and $\Lamt$ can change at each time. To ensure that $\bm{\Sigma}_t$ changes ``slowly", we assume that, when $\P_t$ changes, the eigenvalues along the newly added directions are small initially for the first $d$ frames, and after that they can increase gradually or suddenly to any large value. One precise model for this is specified next.

The model below assumes boundedness of $\lt$. This is more practically valid than the usual Gaussian assumption since most sensor data or noise is bounded. We also replace independence of $\lt$'s by an AR model with independent perturbations $\bnu_t$ and we place the above assumptions on $\bnu_t$. As explained earlier, this is a more practical model and includes independence as a special case.%

\begin{sigmodel}[Model on $\lt$]\label{cor_model} Assume the following.
\ben
\item Let $\bm{\ell}_0=\bm{0}$ and for $t=1,2, \dots t_{\max}$, assume that
\[
\lt = b\bm{\ell}_{t-1} + \nut
\]
for a $b<1$. Assume that the $\nut$ are zero mean, mutually independent and bounded random vectors with covariance matrix
\[
\cov(\nut) = \bm{\Sigma}_{t} \overset{\mathrm{EVD}}{=} \bm{P}_t \bm{\Lambda}_t {\bm{P}_t}'.
\]
%Assume also that the $\nut$'s are independent of all the $\T_{\tilde{t}}$'s for all $\tilde{t}=1,2,\dots,t_{\max}$.???  %\{\T_{\tilde{t}}\}_{\tilde{t}=1,2,\dots,t_{\max}}

%%The $\lt$ are zero mean and bounded random vectors in $\R^n$ that are mutually independent over time. Let $\bm{\Sigma}_t:=\E[\lt{\lt}']$ denote the covariance matrix of $\lt$ at time $t$ and let
%$
%\bm{\Sigma}_t \overset{\mathrm{EVD}}{=} \Pt \Lamt {\Pt}'
%$
%denote its eigenvalue decomposition  (thus $\Pt$ is a basis matrix and $\Lamt$ is diagonal).


\item Let $t_1, t_2, \dots t_J$ denote the subspace change times. The basis matrices $\Pt$  change as
\begin{align*} \label{Pt_def}
\bm{P}_t =
%\begin{cases}
% [\bm{P}_{t-1}  \ \bm{P}_{t,\new}]  & \text{if} \ t = t_1 \text{ or } t_2 \text{ or } \dots \ t_J \\
%\bm{P}_{t-1}  &   \text{otherwise.}
%\end{cases}
%
\begin{cases}
 [(\bm{P}_{t-1} \bm{R}_t \setminus  \bm{P}_{t,\old})  \  \bm{P}_{t,\new}]  & \text{if} \ t = t_1, t_2, \dots \ t_J \\ % \text{ or }
\bm{P}_{t-1}  &   \text{otherwise.}
\end{cases}
%
\end{align*}
where $\bm{R}_t$ is a rotation matrix, $\P_{t_j,\new}$ and $\P_{t_j,\old}$ are basis matrices of size $n \times r_{j,\new}$ and $n \times r_{j,\old}$ respectively, $\bm{P}_{t_j,\old}$ contains a subset of columns of $\bm{P}_{t_j-1} \bm{R}_t$, and $\P_{t_j,\new}{}' \P_{t_j-1} = \bm{0}$ (new directions are orthogonal to previous subspace).

\item Define
\[
\lambda^-:= \lambda_{\min}\left( \frac{1}{t_{\train}}\sum_{t=1}^{t_{\train}} \Lamt \right) \ \text{and} \ \lambda^+:= \lambda_{\max}\left( \frac{1}{t_{\train}}\sum_{t=1}^{t_{\train}} \Lamt \right).
\]
The eigenvalues' matrices $\Lamt$ are such that (i) $\lambda_{\max}(\Lamt) \le \lambda^+ $ and (ii) for a $d< t_{j+1} - t_j$,
%the following holds. Let $\bm{\Lambda}_{t,\new} := {\bm{P}_{t_j,\new}}'\bm{\Sigma}_{t}\bm{P}_{t_j,\new}$ for $t \in [t_j, t_{j+1})$. Assume that
%all their eigenvalues are below $\lambda^+$, and (ii) for the first $d$ frames after a subspace change, the smallest eigenvalue along the newly added directions is large enough to be detectable (is at least $\lambda^-$) and the largest eigenvalue along the newly added directions is not too large (is at most $3\lambda^-$). To be precise, let  Then,
\begin{eqnarray} \label{anew_small}
&& 0< \lambda^- \leq  \lambda_{\new}^-  \leq \lambda_{\new}^+  \leq 3 \lambda^- \  \text{where} \  \nn \\
%\end{eqnarray}
%\begin{eqnarray}
&& \lambda_{\new}^- := \min_j \min_{t\in [t_j,t_j + d]} \lambda_{\min}\left( {\bm{P}_{t_j,\new}}'\bm{\Sigma}_{t}\bm{P}_{t_j,\new} \right), \nn \\
&& \lambda_{\new}^+ := \max_j \max_{t\in [t_j,t_j + d]} \lambda_{\max}\left( {\bm{P}_{t_j,\new}}'\bm{\Sigma}_{t}\bm{P}_{t_j,\new} \right).
%
%&& \lambda^+:= \lambda_{\max}( \frac{1}{t_{\train}}\sum_{t=1}^{t_{\train}} \Lamt), \ \lambda^-:= \lambda_{\min}( \frac{1}{t_{\train}}\sum_{t=1}^{t_{\train}} \Lamt)
%%\lambda^+ &:=& \max_{t} \lambda_{\max}\left( \bm{\Lambda}_{t} \right), \  \lambda^- := \min_{t} \lambda_{\min}\left( \bm{\Lambda}_{t} \right);
\end{eqnarray}

\item Assume that $d\geq(K+2)\alpha$. This also implies that $t_{j+1} - t_{j} > d\geq(K+2)\alpha$. We set $K$ and $\alpha$ in the Theorem. This along with \eqref{anew_small} quantifies ``slow subspace change".


\item Other assumptions: (i) define $t_0:= 1$ and assume that $t_\train \in [t_0, t_1)$;
(ii) for $j=0,1,2, \dots, J$, define
$
r_j: = \rank(\bm{P}_{t_j}) , \ r_{j,\new}:=\rank(\bm{P}_{t_j,\new}), \ r_{j,\old}:=\rank(\bm{P}_{t_j,\old})
$
Clearly, $r_j = r_{j-1}+r_{j,\new} - r_{j,\old}$. Assume that $r_{j,\new}$ is small enough compared to $r_{j,\old}$ so that $r_j \le r$  and $r_{j,\new} \le r_{\new}$ for all $j$ for constants $r$ and $r_\new$. Assume that $r+r_\new < \min(n, t_{j+1}-t_j)$ and $r_\new \leq r_0$. %\footnote{The assumption $r_\new \leq r_0$ is made for simplicity. It can be removed if we assume $\epsilon_w^2 \le 0.03 \zeta \lambda^-$ (remove $r_\new$ in its bound) and do minor changes to the proofs of Lemmas \ref{initsub_cor} and \ref{zetadecay}.}.
%Tighter bounds on $r$ and $r_\new$ are imposed later.
% This ensures that, for all $t > r_J$, the matrix $\bm{L}_t$ is low-rank.
%\item Assume , which is only used in Proof of Lemma \ref{initsub_cor} and Lemma \ref{zetadecay}.

\item Since the $\bnu_t$'s are bounded random variables, there exists a $\gamma< \infty$ and a $\gamma_\new \le \gamma$ such that
\[
\max_t \| \P_t{}' \bnu_t \|_2 \le \gamma, \  \max_j  \max_{t \in[t_j,t_j+d]} \| \P_{t_j,\new}{}' \nut\|_{\infty} \le \gamma_\new.
\]
We assume an upper bound on $\gamma_\new$ in the Thoerem. %This upper bound on $\gamma_\new$ along with  (\ref{anew_small}) and the lower bound on $t_{j+1} - t_{j}$ and $d$ given above quantify ``slow subspace change".


\een
\end{sigmodel}



\begin{figure}
\includegraphics[width=\textwidth]{Figures/Model_Figure_Del.pdf}
\vspace{-0.1in}
\caption{A diagram of Model \ref{cor_model} \label{modelfig}}
\vspace{-0.1in}
\end{figure}

A visual depiction of Model \ref{cor_model} is shown in Figure \ref{modelfig}. The above model is similar to the ones introduced in \cite{rrpcp_perf,rrpcp_isit15}. Various low-rank and ``slow changing" models on $\bm{\Sigma}_t$ are special cases of the above model. One interesting special case is one that allows the variance along new directions to increase slowly as follows: for $t \in [t_j, t_{j}+d]$, let $\Lamtnew:= {\bm{P}_{t_j,\new}}'\bm{\Sigma}_{t}\bm{P}_{t_j,\new}$ and assume that $(\bm{\Lambda}_{t,\new})_{i,i} = (v_i)^{t-t_j} q_i  \lambda^-  \ \text{ for } \ i = 1,\dots,r_{j,\new}$. Here $q_i \ge 1$ and $v_i>1$. An upper bound on $v_i$ of the form $q_i (v_i)^d \leq 3$ ensures that \eqref{anew_small} holds.


\begin{remark} \label{new_eval_inc}
Model \ref{cor_model} requires the upper bound on the eigenvalues along the new directions to hold only for the first $d$ time instants after $t_j$. At any time $t > t_j+d$, the eigenvalues along $\P_{t_j,\new}$ could increase to any large value up to $\lambda^+$ either gradually or suddenly.
\end{remark}




% [see the discussion just below Model 2.1 in \cite{rrpcp_correct}]  the variance along the existing directions to be anything
%
%Notice that, with small modifications to our proof, the condition $\P_t = \P_{t-1}$ for $t \neq t_j$ can be relaxed to $\P_t = [\P_{t-1,*} \bm{R}_{t,*}, \P_{t-1,\new} \bm{R}_{t,\new}$ where $\P_{t-1,*}:= \P_{t_j} \setminus  \P_{t_j,\new}$ and $\P_{t-1,\new}: = \P_{t_j,\new}$ for $t \in [t_j, t_{j+1})$. This means that the existing and new subspaces can keep rotating. ??
%
% $\lambda_{\min}(\Lamt) \ge \lambda^-$ and
% to be the minimum eigenvalue along new directions of any $\alpha$-frame average covariance matrix over the period $[t_j, t_j+d]$

The above model requires the directions to get deleted and added at the same set of times $t=t_j$. This is assumed for simplicity. In general, directions from $\Span(\P_{t_j-1})$ could get deleted at any other time as well. The lower bound in \eqref{anew_small}  requires the energy of $\lt$ along the new directions at {\em all} times $t \in [t_j, t_j+d]$ to be above $\lambda^-$. With very minor changes to the proof (of Lemma \ref{Ak_cor}), we can relax this to the following: we can let $\lambda_\new^-$ be the minimum eigenvalue along the new directions of any $\alpha$-frame {\em average} covariance matrix over the period $[t_j, t_j+d]$ and require this to be larger than $\lambda^-$. For video analytics, this translates to requiring that, after a subspace change, {\em enough (but not necessarily all)} background frames have ``detectable" energy along the new directions, so that the minimum eigenvalue of the average covariance along the new directions is above a threshold. For the recommendation systems' application, this means that the initial set of users may only be influenced by a few, say five, factors, but as more users come in to the system, {\em some (not necessarily all)} of them may also get influenced by a sixth factor (newly added direction).%notationally more complicated to state, but itThis generalization is also more relevant f
%Requiring this to be larger than $\lambda^-$ is weaker than requiring eigenvalues along the new directions to be more than $\lambda^-$ at {\em all} times.

%%
There is a trade off between the upper bound on $\lambda_\new^+$ in \eqref{anew_small} in Model \ref{cor_model} above and the bound on ${\rrho}^2 \beta$ assumed in Model \ref{sbyrho}. Allowing a larger value of $\lambda_\new^+$ will require a tighter bound on $\rho^2\beta$. We chose one set of bounds, but many other pairs would also work. For video analytics, this means that if the background subspace changes are faster, then we also need the foreground objects to be moving more so we can `see' enough of the background behind them. % which corresponds to requiring more changes to $\T_t$

%The mutual independence assumption on $\lt$'s models random background variations around a common mean. This can be easily relaxed be a more general autoregressive model assumption by using matrix Azuma instead of Hoeffding \cite{tail_bound} and adapting ideas from \cite{zhan_reprocs}.


\subsection{Denseness}
To separate sparse $\xt$'s from the $\lt$'s, the basis vectors for the subspace from which the $\lt$'s are generated cannot be sparse. We quantify this using an incoherence condition similar to \cite{rpca}.%
\begin{sigmodel}[Denseness] \label{dense_model}
Let $\mu$ be the smallest real number such that
%\begin{equation}\label{candes_dense}
$
\max_{i} \|{\bm{P}_{t_j}}' \I_i\|_2^2 \leq \frac{\mu r_j}{n}
\ and \
\max_{i} \|{\bm{P}_{t_j,\new}}' \I_i\|_2^2 \leq \frac{\mu r_{j,\new}}{n} \text{ for all } j
$
%\end{equation}
($\I_i$ is the $i^{\text{th}}$ column of the identity matrix; thus $\P'I_i$ is the $i$-th row of $\P$). %(or $i^{\text{th}}$ standard basis vector).
%Recall that $\max_j r_j \le r$ and $\max_j r_{j,\new} \le r_\new$.
Assume that
\[
2s r \mu\leq{0.09n} \text{ and  } 2s r_\new  \mu \leq  {0.0004n}.
\]
\end{sigmodel}

\begin{fact}
Model \ref{dense_model} is one way to ensure that $\|{\bm{P}_{t_j}}' \I_\T\|_2 \le 0.3$ and $\|{\bm{P}_{t_j,\new}}' \I_\T\|_2 \le 0.02$ for all sets $\T$ with $|\T|\le 2s$.
This follows using the fact that for an $r \times s$ matrix $M$, $\|M\|_2 \le \sqrt{s} \max_i \|M_i\|_2$ where $M_i$ is the $i$-th column vector of $M$.
%the spectral norm is upper bounded either by $\sqrt{s}$ times the maximum of $l_2$ norms of any column or by $\sqrt{r}$ times the maximum of $l_2$ norms of any row.
\end{fact}

\subsection{Assumption on the unstructured noise $\wt$} %Assume the following.
%We assume the following on $\wt$ [Model on $\wt$]
%A simple assumption on the unstructured noise  $\wt$ is as follows. %It assumes that $\wt$ is bounded noise, is mutually independent and is also independent of $\x_\tau$ and $\l_\tau$ for all $\tau$. More precisely the following holds.
%Assume that the noise $\wt$ is zero mean and bounded with $\|\wt\|_2 \le \epsilon_w$ (we impose a bound on $\epsilon_w^2$ in the theorem).  Assume also that $\wt, \bm{x}_\tau, \bnu_{\tilde{t}}$ are mutually independent for any $t, \tau, {\tilde{t}}$.
%\item Assume that $\bnu_\tau$ is independent of all $\T_{\tilde{t}}$'s.
%Assume also that the set of random variables $\wt, \bm{x}_\tau, \bnu_\ttau$ for all $t =1,2, \dots t_{\max}$, $\tau=1,2, \dots t_{\max}$, $\ttau=1,2, \dots t_{\max}$, form a set of mutually independent random variables.

\begin{sigmodel}\label{wt_model}
Assume that the noise $\wt$ is zero mean, mutually independent over time, and bounded with $\|\wt\|_2 \le \epsilon_w$. % (we impose a bound on $\epsilon_w$ in the theorem).
%Assume that $\wt$ is independent of all $\T_{\tilde{t}}$'s and $\bnu_{\tilde{t}}$'s\footnote{A clearer way to write this and the independence assumption from Model \ref{cor_model} is as follows: Let $R:=\{\T_{\tilde{t}}\}_{\tilde{t}=1,2,\dots,t_{\max}}$ and assume that the set of random variables $\nut,{t=1,2,\dots,t_{\max}}, \wt, {t=1,2,\dots,t_{\max}} ,R$ are mutually independent.???}.
%$\{\T_{\tilde{t}},\bnu_{\tilde{t}}\}_{\tilde{t}=1,2,\dots,t_{\max}}$.
\end{sigmodel}

%\begin{remark} \label{wt_model_weaker}
%If it is not practical to assume that $\wt$ is independent of $\T_t$ (e.g., if $\wt$ contains the smaller magnitude outlier entries and $\xt$ the larger ones and so $\T_t = \text{support}(\xt)$ cannot be independent of $\wt$), the following assumption can be used with small changes to the proof (see Remark \ref{wt_model_weaker_proof} in Sec. \ref{general_decomp_w}). Let $Q_t:=\{\wt, \T_t\}$. Assume that $\bnu_\tau$ is independent of all $Q_t$'s.
%\end{remark}
%$Q_t$ is independent of all $\bnu_\tau$'s.
%the set of random variables $Q_t, \bnu_\tau$ for all $t =1,2, \dots t_{\max}$, $\tau=1,2, \dots t_{\max}$, are mutually independent.
%are mutually independent over time $t$ and that $Z_t$ and $\bnu_\tau$ are independent for any $t,\tau$.
%Only assume that the pair $\{\wt, \xt\}$ are mutually independent over time $t$ and that they are independent of $\bnu_\tau$ for any $\tau$.

%\begin{remark}
%The above model is the only place where we are treating the $\T_t$'s as random variables. This is needed to ensure that $\lt \wt'$ is close to zero under the appropriate conditioning. %This is also the reason why all the $\T_{\tilde{t}}$'s are included into the random variable $X_u$ defined in Definition \ref{def_X}. This is the random variable that we condition on each time we apply the matrix Azuma inequality.
%For the special case of our result where $\wt=0$, we need not treat the $\T_t$'s as random variables.
%%We actually only need this assumption on $\T_t$'s (support of $\xt$'s).
%\end{remark}


%The above model is simple but it does not allow for $\wt$ to be the modeling error due to either $\xt$ containing small entries or due to the $\lt$'s not forming a low-rank matrix. In the first case, $\wt$ and $\xt$ will not be independent, while in the second case, $\wt$ and $\lt$ will not be independent. A more general model that allows this and includes Model \ref{wt_model_0} as a special case is the following.
%\begin{sigmodel}\label{wt_model}
%(1) The noise $\wt$ is zero mean, bounded and mutually independent over time and satisfies $\|\wt\|_2 \le \epsilon_w$ (we impose a bound on $\epsilon_w^2$ in the theorem). %$\epsilon_w^2 \le \sigma_w^2$
%(2) It can be split into $\wt = \wt^x + \wt^\ell$ where $\wt^x$ is such that
%$\lt$ is independent of $\{ \wt^x , \xt\}$;
%and $\wt^\ell$ is such that $\xt$ is independent of $\{ \wt^\ell , \lt\}$ and, $\wt^\ell$ and $\lt$ are uncorrelated, i.e., $\E[\lt \wt']=0$. % %for any $t,\tau$, $\wt^\ell$ and $\l_\tau$ are uncorrelated.
%%
%%$\ell_t$ is independent of $\{\xt, \wt^x\}$ and $\xt$ is independent of $\{\lt, \wt^\ell\}$.
%%and $\|\E[w_t w_t']\|_2 \le \sigma_w^2$.  %| \T_t
%\end{sigmodel}
%%\begin{sigmodel}\label{wt_model}
%%(1) The noise $\wt$ is zero mean, bounded and mutually independent over time and satisfies $\|\wt\|_2 \le \epsilon_w$ (we impose a bound on $\epsilon_w^2$ in the theorem). %$\epsilon_w^2 \le \sigma_w^2$
%%(2) It can be split into $\wt = \wt^x + \wt^\ell$ where $\wt^x$ is such that
%%$\bnu_t$ is independent of $\{ \wt^x , \xt\}$;
%%and $\wt^\ell$ is such that $\xt$ is independent of $\{ \wt^\ell , \bnu_t\}$ and, for any $t,\tau$, $\wt^\ell$ and $\bnu_\tau$ are uncorrelated.
%%%
%%%$\ell_t$ is independent of $\{\xt, \wt^x\}$ and $\xt$ is independent of $\{\lt, \wt^\ell\}$.
%%%and $\|\E[w_t w_t']\|_2 \le \sigma_w^2$.  %| \T_t
%%\end{sigmodel}
%%The above model is one way to ensure that (a) $\E[\lt \wt'|\T_t] = 0$ and (b) $\|\E[\wt \wt'|\T_t]\|_2 \le \sigma_w^2$. These two facts are used in our proofs.
%
%\begin{fact} \label{wt_fact}
%Model \ref{wt_model} is one way to ensure that $\wt$ is zero mean, bounded, and mutually independent over time, and is such that (a) $\E[\lt \wt'|\T_t] = 0$ and (b) $\|\E[\wt \wt'|\T_t]\|_2 \le \epsilon_w^2$.
%\end{fact}


\subsection{Main result for Automatic ReProCS} \label{noclust_result} % (Algorithm \ref{cPCA_algo})
In this section, we give a correctness result for Automatic ReproCS, i.e., for Algorithm \ref{reprocsdet} with the cluster PCA (cPCA) step removed. This is exactly the algorithm studied in our earlier work \cite{rrpcp_isit15}. The result given in \cite{rrpcp_isit15} for it required mutual independence of the $\lt$'s over time. For the video application, this means that background changes at different times are due to independent causes, e.g., independent light flickers. This is often a restrictive assumption. The current result replaces this requirement with an autoregressive model which is a much better model for background changes due to correlated factors such as moving lake or sea waters.
%since most backgrounds, e.g., moving waters, involve correlated changes over time.

The main idea of Automatic ReProCS is as follows.  It estimates the initial subspace as the top $r_0$ left singular vectors of $[\bm{m}_1,\bm{m}_2,\dots, \bm{m}_{t_\train}]$. %Let $\Phat_t$ denote the basis matrix for the subspace estimate at time $t$.
At time $t$, if the previous subspace estimate, $\Phat_{t-1}$, is accurate enough, because of the ``slow subspace change" assumption, projecting $\mt = \xt + \lt + \wt$ onto its orthogonal complement nullifies most of $\lt$. Specifically, we compute $\bm{y}_t:= \bm{\Phi}_t \mt$ where $\bm{\Phi}_t:= \I - \Phat_{t-1}\Phat_{t-1}{}'$. Clearly, $\bm{y}_t = \bm{\Phi}_t \xt + \bm{b}_t$ with $\| \bm{b}_t \|_2$ being small. %: $\| \bm{\Phi}_t\lt\|_2$  is small due to the slow subspace change assumption and $\|\wt\|_2 \le \epsilon_w$.
Thus recovering $\xt$ from $\bm{y}_t$ is a traditional sparse recovery problem in small noise \cite{candes_rip}. We recover $\xt$ by $l_1$ minimization with the constraint $\| \bm{y}_t - \bm{\Phi}_t x\|_2 \le \xi$ and estimate its support by thresholding using a threshold $\omega$. We use the estimated support, $\That_t$, to get an improved debiased estimate of $\xt$, denoted $\xhatt$, by least squares (LS) estimation on $\That_t$ \cite{dantzig}. We then estimate $\lt$ as $\lhat_t = \mt - \xhatt$. %By the denseness assumption given in Model \ref{dense_model}, it can be argued that the restricted isometry constant (RIC) of $\bm{\Phi}_t$ will be small. Under the theorem's assumptions, we can bound it by 0.14. This ensures that a sparse $\xt$ is indeed accurately recoverable from $\bm{y}_t$.
%
The estimates $\lhatt$ are used in the subspace estimation step which involves (i) detecting subspace change; and (ii) $K$ steps of projection-PCA, each done with a new set of $\alpha$ frames of $\lhatt$, to get an accurate enough estimate of the new subspace. This step is explained in detail later in Sec. \ref{algo_sec}. %Since cPCA is not called, this does not delete old directions from the subspace estimate.
Automatic ReProCS has four algorithm parameters - $\alpha$, $K$, $\xi$, $\omega$ - whose values will be set in the result below.
%; and (iii) cluster PCA to delete the old subspace by re-estimating the current subspace. At the end of the projection PCA step, the estimated subspace dimension is at most $r+r_\new$, and after cluster PCA, it comes down to at most $r$.


%Automatic ReproCS without cPCA has four parameters - $\alpha$, $K$, $\xi$, $\omega$ - that need to be set appropriately. The parameter $\alpha$ is the number of consecutive time instants that are used to obtain {\em an} estimate of the new subspace, and $K$ is the total number of times the new subspace is estimated before we get an accurate enough estimate of it. The parameter $\xi$ is the bound on the $l_2$ norm of the noise seen by the projected sparse recovery step, and $\omega$ is the threshold used to recover the support of $\xt$. %The parameter $\ghatp$ is used to estimate the eigenvalue clusters automatically from an empirical covariance matrix computed using an appropriate set of $\lhatt$'s.



%
%\begin{definition}Define
%$\gamma:= \sup_t \|{\bm{P}_{t}}'\nut\|_{\infty}$,  $\gamma_\new:= \max_j  \max_{t \in[t_j,t_j+d]} \| \P_{t_j,\new}{}' \nut\|_{\infty}$ and $b_0=0.1$.
%\end{definition}

\begin{theorem}\label{thm1_cor_nodel}
Consider Algorithm \ref{reprocsdet} without the cluster PCA step.
Assume that, for $t > t_\train$, $\mt = \lt + \wt + \xt$ and, for $t \le t_\train$,  $\mt = \lt + \wt$.
Pick a $\zeta$ that satisfies %\frac{\lambda^-}{(r+r_\new)^3\gamma^2},
\[
\zeta \leq \min \left\{ \frac{10^{-4}}{(r_0+Jr_\new)^2} , \frac{0.003\lambda^-}{(r_0+Jr_\new)^2 \lambda^+} , \frac{1}{(r_0+Jr_\new)^3\gamma^2}, \frac{0.05\lambda^-}{(r_0+Jr_\new)^3\gamma^2} \right\}.
\]
%(Notice that for $(r+r_\new)\geq 20$, the last bound will already be satisfied by the fourth bound.)
Let $b_0=0.1$.
Suppose that the following hold.
\begin{enumerate}

\item enough initial training data is available: $t_\train \ge \frac{32 (2(r_0+Jr_\new) \gamma^2)^2}{ (1-b_0)^2 (0.001 r_\new\zeta \lambda^-)^2} (11 \log n + \log 8) $

\item algorithm parameters are set as:
\\ $\xi =  \xi_{\mathrm{cor}} := \epsilon_w + \frac{2\sqrt{\zeta} + \sqrt{r_{\new}}\gamma_{\new}}{1-b_0}$; $\omega = 7\xi$;  $K = \left\lceil \frac{\log(0.85r_\new\zeta)}{\log(0.2)}\right\rceil$;
\\ $\alpha = \alpha_{\add}$ where
$
\alpha_{\add}  \ge  32 \frac{1.2^2 (2\sqrt{\zeta} + \sqrt{r_\new}\gamma_\new + 2\epsilon_w)^4}{(1-b_0)^6} \frac{(1-b_0^2)^2}{(0.001 r_\new \zeta\lambda^-)^2} (11 \log n + \log ((52K+44)J) ) %???
$
%%{32\cdot100^2}\frac{\max\{32 , 1.2(\sqrt{\zeta} + \sqrt{r_\new}\gamma_\new + \epsilon_w)^4\}}{ \left(r_\new \zeta \lammin \right)^2} (\log(6(K+1)J) + 11\log n )$
%and
%$\alpha_{\del}  \ge  \frac{8 \cdot 3 (r \gamma^2)^2}{ (0.01r_{\new}\zeta \lambda^-)^2} (\log (6 (\vartheta+1) J) + 11 \log n);$

\item model on $\T_t$: Model \ref{sbyrho} holds; %(recall that we need ${\rrho}^2 \beta \leq  0.01 \alpha$)

%%$\bm{R}_t=\I$,
\item model on $\lt$:
\\ Model \ref{cor_model} holds with $\P_{t_j,\new}{}' [\P_0, \P_{t_1,\new}, \P_{t_2,\new}, \dots \P_{t_{j-1},\new}] = \bm{0}$, $b \le b_0=0.1$, and with $\sqrt{r_\new}\gamma_{\new}$ small enough so that $14 \xi \le \min_{t} \min_{i \in \T_t} |(x_t)_i|$;
%\\ Model \ref{clust_model} holds with $|\mathcal{G}_{j,k}| \ge 0.27 (r+r_\new)$; %r_{j,k}:=
\\ Model \ref{dense_model} (denseness) holds with $r$ replaced by $(r_0+Jr_\new)$.
%(recall that we need $ 2rs \mu \le 0.09n$ and $2r_\new s \mu \le 0.0004n$);
%\\ $b^2r_{\new}\eta_{\new}\lambda_{\new}^+ \leq 0.5\lambda^-$ (because $b\leq0.1$, this will be satisfied if $r_{\new}\eta_{\new}\lambda_{\new}^+ \leq 50\lambda^-$); ?? may or may not need this
\label{xmin_cond}

\item model on $\wt$: Model \ref{wt_model} holds with $\epsilon_w^2 \le 0.03\zeta  \lambda^-$ % %\ref{wt_model_cor} holds with
%(this also ensures that the initial subspace estimate is accurate enough: $\mathrm{dif}( \Phat_{\ttrain}, \bm{P}_{\ttrain} ) \le \frac{0.03 \zeta}{1-0.03 \zeta} \le 0.04 \zeta \le r_0 \zeta$)

\item independence: Let $\T:=\{\T_{\tilde{t}}\}_{\tilde{t}=1,2,\dots,t_{\max}}$.
Assume that $\T,  \bm{w}_1, \bm{w}_2, \dots, \bm{w}_{t_{\max}}, \bnu_1, \bnu_2, \dots, \bnu_{t_{\max}}$ are mutually independent random variables. %???
\label{indep_cond}
%$\{\T_{\tilde{t}},\bnu_{\tilde{t}}\}_{\tilde{t}=1,2,\dots,t_{\max}}$

%Assume that $\wt$ is independent of all $\T_{\tilde{t}}$'s and $\bnu_{\tilde{t}}$'s\footnote{A clearer way to write this and the independence assumption from Model \ref{cor_model} is as follows: Let $R:=\{\T_{\tilde{t}}\}_{\tilde{t}=1,2,\dots,t_{\max}}$ and assume that the set of random variables $\nut,{t=1,2,\dots,t_{\max}}, \wt, {t=1,2,\dots,t_{\max}} ,R$ are mutually independent.???}.
%$\{\T_{\tilde{t}},\bnu_{\tilde{t}}\}_{\tilde{t}=1,2,\dots,t_{\max}}$.


\end{enumerate}
Then, with probability  $\ge 1 - 2n^{-10}$, at all times $t$,
\ben
\item $\T_t$ is exactly recovered, i.e. $\hat{\T}_t = \T_t$ for all $t$;
\item  $\|\xt - \xhatt\|_2 \le  1.34 \left(2\sqrt{\zeta} +  \sqrt{r_\new}\gamma_{\rmnew}  + \epsilon_w  \right)$ and $\|\lhat_t - \lt \|_2 \le \|\xt - \xhatt\|_2 + \epsilon_w$;
\item the subspace error $\SE_t := \|( \I - \hat{\bm{P}}_t \hat{\bm{P}}_t{}' ) \Pt \|_2 \le 10^{-2} \sqrt{\zeta}$ for all $t\in[t_{j}+d,t_{j+1})$.
%
\item the subspace change time estimates satisfy $t_j \leq \hat{t}_j \leq t_j + 2\alpha$; and its estimates of the number of new directions are correct: $\hat{r}_{j,\new,k} = r_{j,\new}$ for $j=1,\dots,J$.% and $k = 1,\dots,K$.

%\item  eigenvalue clusters are recovered exactly: $\hat{\mathcal{G}}_{j,k} = \mathcal{G}_{j,k}$ for all $j$ and $k$; thus the its estimate of number of deleted directions is also correct.
    %$\hat{r}_j = \sum_{k=1}^{\vartheta_j} |\hat{\mathcal{G}}_{j,k}|$ and $\hat{r}_{j,\old} =
    %($\hat{r}_{j,old} = \hat{r}_{j-1} - \sum_{k=1}^{\vartheta_j} |\hat{\mathcal{G}}_{j,k}|$ and $\hat{r}_{j} =\hat{r}_{j,\new}+\sum_{k=1}^{\vartheta_j} |\hat{\mathcal{G}}_{j,k}|$
\een
\end{theorem}

{\em Proof: } The above result follows as a corollary of the more general result, Theorem \ref{thm1_cor}, that is given below. For its proof, please see Appendix \ref{proof_thm1_cor_nodel}.

\begin{remark} \label{wt_model_weaker}
Consider condition \ref{indep_cond}). If it is not practical to assume that $\wt$'s are independent of $\T$ (e.g., if $\wt$ contains the smaller magnitude outlier entries and $\xt$ the larger ones and so $\T_t = \text{support}(\xt)$ cannot be independent of $\wt$), the following weaker assumption can be used with small changes to the proof (see Fact \ref{wt_model_weaker_proof} in Sec. \ref{general_decomp_w}). Let $Q:=\{\T,\{\wt\}_{t=1,2,\dots,t_{\max}}\}$. Assume that $Q, \bnu_1, \bnu_2, \dots, \bnu_{t_{\max}}$ are mutually independent.
\end{remark}


%: $\|\wt\|_2 \le \epsilon_w$ with $\epsilon_w$ small enough;
Theorem \ref{thm1_cor_nodel} says the following. If an accurate estimate of the initial subspace is available ($t_\train$ is large enough); the algorithm parameters are set appropriately;  the outlier support at time $t$, $\T_t$, has enough changes over time; $\lt$ follows an AR model with parameter $b \le b_0=0.1$ (i.e., the $\lt$'s are not too correlated over time); the low-dimensional subspace from which $\bnu_t$ is generated (this is also approximately the subspace from which $\lt$ is generated) is fixed or changes ``slowly" enough, i.e. (i) the delay between change times is large enough ($t_{j+1}-t_j > d \ge (K+2)\alpha$) and (ii) the eigenvalues along the newly added directions are small enough for $d$ frames after a subspace change; the basis vectors whose span defines the low-dimensional subspaces are dense enough; the noise $\wt$ is small enough; then, with high probability (whp), the error in estimating $\lt$ or $\xt$ will be bounded by a small value at all times $t$. Also, whp, the outlier support will be exactly recovered at all times; and the error in estimating the low-dimensional subspace will decay to a small constant times $\sqrt{\zeta}$ within a finite delay of a subspace change.  Moreover, subspace changes will get detected within a short delay, and the dimension of the newly added subspaces will get correctly estimated.

The condition ``$14 \xi \le \min_{t} \min_{i \in \T_t} |(x_t)_i|$" in condition \ref{xmin_cond}) can be interpreted either as another slow subspace change condition or as a requirement that the minimum magnitude nonzero entry of $\xt$ (the smallest magnitude outlier) be large enough compared to $\epsilon_w + \sqrt{r_\new} \gamma_\new$. Interpreted this way, it says the following. If $\lt$ is the true data, $\mt-\lt = \wt+\xt$ is the vector of corruptions with $\wt$ being the small corruptions and the nonzero entries of $\xt$ being the large ones (outliers). We need $\wt$ to be small enough to not affect subspace recovery error too much ($\|\wt\|_2 \le \epsilon_w \le \sqrt{0.03 \zeta \lambda^-}$) and we need the nonzero entries of $\xt$ to be large enough  to be detectable ($\min_{t} \min_{i \in \T_t} |(x_t)_i| \ge 14 \xi \approx 14(\epsilon_w + \sqrt{r_\new} \gamma_\new)$). %???
%they needs to be large compared to the energy in the small corruptions plus the energy in the newly added subspace:

%This is relevant for applications such as understanding dynamic social networks' structural changes in the presence of outliers. While many heuristics exist to detect sudden subspace changes, our algorithm and result provides an approach for detecting and tracking slow subspace changes.% (slow changes)for a period of time after the previous subspace change has stabilized, the eigenvalues of $\cov(\lt)$ are ``clustered";


%We assume that for a period of time before the next subspace change, the eigenvalues along the existing directions
\subsection{Eigenvalues' clustering assumption and main result for Automatic ReProCS-cPCA}  \label{clust_result}

The ReProCS algorithm studied above (which is the same as the one introduced in \cite{rrpcp_isit15}) does not include a step to delete old directions from the subspace estimate. As a result, its estimated subspace dimension can only increase over time. This necessitates a bound on the number of subspace changes, $J$. The bound is imposed by the denseness assumption - notice that Theorem \ref{thm1_cor_nodel} requires the bound in Model \ref{dense_model} to hold with $r$ replaced by $r_0+Jr_\new$. In this section, we relax this requirement by analyzing automatic ReProCS-cPCA (Algorithm \ref{reprocsdet}) which includes cluster PCA to delete the old directions from the subspace estimate. This is done by re-estimating the current subspace.

In order to be able to design an accurate algorithm to delete the old directions by re-estimating the current subspace, we need one of the following  for a period of $d_2$ frames within the interval $[t_j,t_{j+1})$. We either need the condition number of $\Lamt$ (or equivalently of $\bm\Sigma_{t}$) to be small, or we need a generalization of it: we need its eigenvalues to be ``clustered" into a few (at most $\vartheta$) clusters in such a way that the condition number within each cluster is small and the distance between consecutive clusters is large (clusters are well separated). %(the smallest eigenvalue of cluster $k$ is much larger than the largest eigenvalue of cluster $k+1$).
The problem with requiring a small upper bound on the condition number of $\bm\Sigma_t$ is that it disallows situations where the $\lt$'s constitute large but structured noise. This is why the ``clustered" generalization is needed. This would be valid for data that has variations at different scales. For example, for data that has variations at two scales, there would be two clusters, the large scale variations would form the first cluster and the small scale ones the second cluster. These clusters would naturally be well separated.

Let $\vartheta$ denote the maximum number of clusters. As we will explain in Sec. \ref{algo_sec}, the subspace deletion via re-estimation step is done after the new directions are accurately estimated. As explained later, with high probability (whp), this will not happen until $t_j+K \alpha$. Thus, we assume that the clustering assumption holds for the period $[t_j+K \alpha+1, t_j+K \alpha+d_2]$ with $d_2 > (\vartheta+3)\alpha$ and $t_{j+1}-t_j > K \alpha + d_2$. In the algorithm, cluster PCA is done starting at $\that_j + K \alpha$.

\begin{sigmodel} \label{clust_model}
Assume the following.
\ben
\item Assume that $t_{j+1} - t_j > K \alpha + d_2$ for an integer $d_2 \ge (\vartheta+3)\alpha$ (where $\vartheta$ is defined below). Assume that for all $t \in [t_j+K \alpha+1, t_j+K \alpha+d_2]$, $\Lamt$ is constant; let $\Lamj$ be this constant matrix and assume that $\lambda_{\min}(\Lamj) \ge \lambda^-$.

\item Define a partition of the index set $\{1,2, \dots r_{j} \}$ into sets $\mathcal{G}_{j,1}, \mathcal{G}_{j,2}, \dots , \mathcal{G}_{j,\vartheta_j}$ as follows. Sort the eigenvalues of $\bm{\Lambda}_{(j)}$ in decreasing order of magnitude. To define $\mathcal{G}_{j,1}$, start with the first (largest) eigenvalue and keep adding smaller eigenvalues to the set. Stop when the ratio of the maximum to the minimum eigenvalue first exceeds $g^+ = 3$ or when there are no more nonzero eigenvalues.
Suppose this happens for the $i$-th eigenvalue. Then, define $\mathcal{G}_{j,1} = \{1,2, \dots i-1\}$. For  $\mathcal{G}_{j,2}$, start with the $i$-th eigenvalue and repeat the same procedure. Keep doing this until there are no more nonzero eigenvalues. Let $\vartheta_j$ denote the number of clusters for the $j$-th subspace and let $\vartheta:= \max_j \vartheta_j$.
Define
\[
\lambda_{j,k}^+:= {\max_{i\in\mathcal{G}_{j,k}}\lambda_i\left(\bm{\Lambda}_{(j)}\right)}, \ \ \lambda_{j,k}^-:= {\min_{i\in\mathcal{G}_{j,k}}\lambda_i\left(\bm{\Lambda}_{(j)}\right)}
\]

Assume that the clusters are well-separated, i.e., %``clustered" (distance between the sets $\mathcal{G}_{j,k}$ is large enough), i.e.,
 \begin{equation}\label{chi}
\frac{\lambda_{j,k+1}^+}{\lambda_{j,k}^-} \le {\chi}^+ = 0.2
 %\frac{\max_{i\in\mathcal{G}_{j,k+1}}\lambda_i\left(\bm{\Lambda}_{(j)}\right) }{\min_{i\in\mathcal{G}_{j,k}}\lambda_i\left(\bm{\Lambda}_{(j)}\right)} \le {\chi}^+ = 0.2
 \end{equation}
%For ease of notation, henceforth, we will assume that there are $\vartheta$ clusters for all $j$. If $\vartheta_j < \vartheta$, it will just mean that the last $(\vartheta - \vartheta_j+1)$ clusters are empty.
\een
\end{sigmodel}

\begin{fact}
The above way of defining the clusters is one way to ensure that the condition number of the eigenvalues within each cluster (ratio of the maximum to minimum eigenvalue of the cluster) is below $g^+ = 3$, i.e.,
for all $k=1,2,\dots, \vartheta_j$,
\begin{equation}\label{gjk}
\frac{\lambda_{j,k}^+}{\lambda_{j,k}^-} \le g^+ = 3.
%\frac{\max_{i \in \mathcal{G}_{j,k}} \lambda_i( \bm{\Lambda}_{(j)} )}{\min_{i \in \mathcal{G}_{j,k}} \lambda_i( \bm{\Lambda}_{(j)}  )} \le g^+ = 3.
\end{equation}
\end{fact}

A model similar to Model \ref{clust_model} was first introduced in \cite{rrpcp_perf} where the cluster PCA idea was introduced.
%More precisely, for every   $u = \lceil \frac{t_{j+1}-d_2}{\alpha} \rceil +1, \lceil \frac{t_{j+1}-d_2}{\alpha} \rceil + 2, \dots \lceil \frac{t_{j+1}}{\alpha} \rceil - 1$, $\bm{\Lambda}_{(j)}^u:= \frac{1}{\alpha} \sum_{t \in (u-1)\alpha+1}^{u \alpha} \Lamt$ satisfies $\lambda_{\min}(\bm{\Lambda}_{(j)}^u) \ge \lambda^-$ and satisfies the condition given in (2) in the model above.

\begin{remark}
The case when, for the entire period  $[t_j+K \alpha+1, t_j+K \alpha+d_2]$, the condition number of $\bm\Sigma_t$ is below $g^+$ is a special case of Model \ref{clust_model} with $\vartheta_j=\vartheta=1$ and $\chi^+ = 0$.
\end{remark}


\begin{remark}\label{new_eval_inc_2}
Model \ref{cor_model} requires the eigenvalues along $\P_{t_j,\new}$ to be small for $t \in [t_j, t_j+d]$ with $d \ge (K+2)\alpha$ while  Model \ref{clust_model} requires all eigenvalues to be constant for $t \in [t_j+K \alpha+1, t_j+K \alpha+d_2]$.
%of $\Lamtnew$ to be small (below $3\lambda^-$). Recall that $\Lamtnew = \P_{t_j,\new}{}' \Lamt \P_{t_j,\new}$ for $t \in [t_j, t_{j+1}-1]$.
Taken together, this means that for all $t \in [t_j, t_j+K \alpha+d_2]$, we are requiring that the eigenvalues along $\P_{t_j,\new}$ be small. However after $t=t_j+K \alpha+d_2$, there is no constraint on its eigenvalues until $t=t_{j+1}+K \alpha$ at which time Model \ref{clust_model} again requires all eigenvalues to be constant.
Thus, in the interval $[t_j+K \alpha+d_2+1, t_{j+1}+K \alpha]$, or in later intervals of the form  $[t_{j+j'}+K \alpha+d_2+1, t_{j+j'+1}+K \alpha]$ for any $j'>0$, the eigenvalues along $\P_{t_j,\new}$ could increase to any large value up to $\lambda^+$ either gradually or suddenly. Or they could also decrease to any small value.
%By $t= t_{j+1}+K \alpha+1$ some, or all, eigenvalues along $\P_{t_j,\new}$ could have increased to $\lambda^+$ or decreased to zero or be anything in between.
\end{remark}
%Model \ref{cor_model} requires the upper bound on the eigenvalues along the new directions to hold only for the first $d$ time instants after $t_j$. At any time $t > t_j+d$, the eigenvalues along $\P_{t_j,\new}$ could increase to any large value up to $\lambda^+$ either gradually or suddenly.

%Then $\that_j+d \le t_j+(K+5)\alpha$.
%\begin{remark}

With small changes to the proof, one can relax the $\Lamt$ constant requirement to the following. Let $\mathrm{ClustInterval}$ denote the interval $[t_j+K\alpha+ 1, t_j+K\alpha +d_2]$ %or the interval $[t_j+K\alpha + 3\alpha+ \Delta+ 1, t_j+K\alpha + 3\alpha+ \Delta +d_2]$ (if using the above relaxation)
and let $t_0$ denote the first time instant of $\mathrm{ClustInterval}$.
Define a partition of the index set $\{1,2, \dots r_{j} \}$ into sets $\mathcal{G}_{j,1}, \mathcal{G}_{j,2}, \dots , \mathcal{G}_{j,\vartheta_j}$ as in Model \ref{clust_model} but by using $\bm\Lambda_{t_0}$ to replace $\Lamj$.
Assume that for all $k=1,2,\dots, \vartheta_j$,
$\lambda_{j,k}^- \le \min_{i \in \mathcal{G}_{j,k}} \min_{t \in \mathrm{ClustInterval}} \lambda_i( \bm{\Lambda}_{t}) \le \max_{i \in \mathcal{G}_{j,k}} \max_{t \in \mathrm{ClustInterval}} \lambda_i( \bm{\Lambda}_{t}) \le \lambda_{j,k}^+.$
%$\frac{\max_{i \in \mathcal{G}_{j,k}} \max_{t \in \mathrm{ClustInterval}} \lambda_i( \bm{\Lambda}_{t} )}{\min_{i \in \mathcal{G}_{j,k}} \min_{t \in \mathrm{ClustInterval}} \lambda_i( \bm{\Lambda}_{t}  )} \le g^+ = 3 $ and $\frac{\max_{i\in\mathcal{G}_{j,k+1}} \max_{t \in \mathrm{ClustInterval}}\lambda_i\left(\bm{\Lambda}_{t}\right) }{\min_{i\in\mathcal{G}_{j,k}} \min_{t \in  \mathrm{ClustInterval}}\lambda_i\left(\bm{\Lambda}_{t}\right)} \le {\chi}^+ = 0.2$.
%\end{remark}


At the cost of making our model more complicated, the requirement discussed in Remark \ref{new_eval_inc_2} can also be relaxed, i.e., we can allow the eigenvalues along $\P_{t_j,\new}$ to increase to a large value before imposing Model \ref{clust_model}. To do this we need to assume an upper bound on $d$. Suppose that $(K+2)\alpha \le d \le (K+3)\alpha$. Suppose also that we allow a period of $\Delta = 4 \alpha$ frames for the new eigenvalues to increase. We can assume Model \ref{clust_model} holds for the period $[t_j+K\alpha + 3\alpha+ \Delta+ 1, t_j+K\alpha + 3\alpha+ \Delta +d_2]$ with $d_2> (\vartheta+3)\alpha$. In addition, we would also need $t_{j+1}-t_j >(K+3)\alpha+\Delta+d_2$. With this, we would run the cluster PCA algorithm starting at $\that_j+K\alpha + 3\alpha+ \Delta$ instead of at $\that_j+K\alpha$ as we do now.
%With these minor changes, all our proofs will apply without change.
%\end{remark}




We give below a correctness result for Automatic ReproCS-cPCA (Algorithm \ref{reprocsdet}) that uses the above model. It has one extra parameter, $\ghatp$, other than the four used by Automatic ReProCS. $\ghatp$ is used to estimate the eigenvalue clusters automatically from an empirical covariance matrix computed using an appropriate set of $\lhatt$'s.
%It has five parameters - $\alpha$, $K$, $\xi$, $\omega$, $\ghatp$ - that need to be set appropriately. The parameter $\alpha$ is the number of consecutive time instants that are used to obtain {\em an} estimate of the new subspace, and $K$ is the total number of times the new subspace is estimated before we get an accurate enough estimate of it. The parameter $\xi$ is the bound on the $l_2$ norm of the noise seen by the projected sparse recovery step of the algorithm, and $\omega$ is the threshold used to recover the support of $\xt$. The parameter $\ghatp$ is used to estimate the eigenvalue clusters automatically from an empirical covariance matrix computed using an appropriate set of $\lhatt$'s.

%\begin{definition}Define
%$\gamma:= \sup_t \|{\bm{P}_{t}}'\nut\|_{\infty}$, $\gamma_\new:= \max_j  \max_{t \in[t_j,t_j+d]} \| \P_{t_j,\new}{}' \nut\|_{\infty}$ and $b_0=0.1$.
%\end{definition}

\begin{theorem}\label{thm1_cor}
Consider Algorithm \ref{reprocsdet}.
%Let $r_\new := \max_j r_{j,\new}$, $r = \max_j r_j$. %Recall that $\gamma:=\max_t \|{\bm{P}_t}' \nut\|_{\infty}$ and $\gamma_\new:=\max_j \max_{t \in [t_j, t_{j}+d)} \|{\bm{P}_{t_j,\new}}'\nut \|_{\infty}$.
%Assume that $\mt$ satisfies \eqref{orpca_eq} with $\xt=0$ for $t \le t_\train$.
%
Assume that, for $t > t_\train$, $\mt = \lt + \wt + \xt$ and, for $t \le t_\train$,  $\mt = \lt + \wt$.
Pick a $\zeta$ that satisfies %\frac{\lambda^-}{(r+r_\new)^3\gamma^2},
\[
\zeta \leq \min \left\{ \frac{10^{-4}}{(r+r_\new)^2} , \frac{0.003\lambda^-}{(r+r_\new)^2 \lambda^+} , \frac{1}{(r+r_\new)^3\gamma^2}, \frac{0.05\lambda^-}{(r+r_\new)^3\gamma^2} \right\}.
\]
%(Notice that for $(r+r_\new)\geq 20$, the last bound will already be satisfied by the fourth bound.) $r \ge 4$ and
Let $b_0=0.1$.
Suppose that the following hold.
\begin{enumerate}

\item enough initial training data is available: $t_\train \ge \frac{32 (2r \gamma^2)^2}{ (1-b_0)^2 (0.001 r_\new\zeta \lambda^-)^2} (11 \log n + \log 8)$
%$t_\train \ge \frac{\max( 3r \gamma^2, 3\epsilon_w^2)}{0.01 \zeta^2 \lambda^-} (11 \log n + \log 4)$ ?? edit the numbers;
%\frac{11 \cdot 8 \max( r \gamma^2, \epsilon_w^2)^2}{(\zeta \lambda^-)^2} \log n$

\item algorithm parameters are set as:
\\ $\xi =  \xi_{\mathrm{cor}} := \epsilon_w + \frac{2\sqrt{\zeta} + \sqrt{r_{\new}}\gamma_{\new}}{1-b_0}$; $\omega = 7\xi$;  $K = \left\lceil \frac{\log(0.85r_\new\zeta)}{\log(0.2)}\right\rceil$; $\ghatp: =  \frac{g^+ + 0.06}{1-0.06}  = 3.26$;
\\ $\alpha = \max\{\alpha_{\add},\alpha_{\del}\}$ where
$
\alpha_{\add}  \ge  32 \frac{1.2^4 (2\sqrt{\zeta} + \sqrt{r_\new}\gamma_\new + 2\epsilon_w)^4}{(1-b_0)^6} \frac{(1-b_0^2)^2}{(0.001 r_\new \zeta\lambda^-)^2} (11 \log n + \log ( (52K+44)J) )
$
%{32\cdot100^2}\frac{\max\{32 , 1.2(\sqrt{\zeta} + \sqrt{r_\new}\gamma_\new + \epsilon_w)^4\}}{ \left(r_\new \zeta \lammin \right)^2} (\log(6(K+1)J) + 11\log n )$
and
$\alpha_{\del} \ge 32 \frac{1.2^4 r^2\gamma^4}{(1-b_0)^6} \frac{(1-b_0^2)^2}{(0.001 r_\new \zeta\lambda^-)^2} (11 \log n + \log ( (52\vartheta+36)J) );$
%$\alpha_{\del} \ge 32 \frac{1.2^4 (2\sqrt{\zeta} + \sqrt{r_\new}\gamma_\new + 2\epsilon_w)^4}{(1-b_0)^6} \frac{(1-b_0^2)^2}{(0.001 r_\new \zeta\lambda^-)^2} (11 \log n + \log ( (52\vartheta+36)J) );$ ???
%\frac{8 \cdot 3 (r \gamma^2)^2}{ (0.01r_{\new}\zeta \lambda^-)^2} (\log (4 (\vartheta+1) J) + 11 \log n)

%\item $0.8\lambda^- \leq \lamtrain \leq 1.2\lambda^-$

\item model on $\T_t$: Model \ref{sbyrho} holds; %(recall that we need ${\rrho}^2 \beta \leq  0.01 \alpha$)


%$\ds\vartheta_{j}\leq \frac{3.8r_{(j)}}{r+r_\new}$;  $d \geq(K+2)\alpha$ $d_2\geq(\max_j \vartheta_j+3)\alpha$ and

\item model on $\lt$:
\\ Model \ref{cor_model} holds with $b \le b_0=0.1$ and with $\sqrt{r_\new}\gamma_{\new}$ small enough so that $14 \xi \le \min_{t} \min_{i \in \T_t} |(x_t)_i|$;
\\ Model \ref{clust_model} holds with $|\mathcal{G}_{j,k}| \ge 0.15 (r+r_\new) $; %r_{j,k}:=???
\\ Model \ref{dense_model} (denseness) holds. %(recall that we need $ 2rs \mu \le 0.09n$ and $2r_\new s \mu \le 0.0004n$);
%\\ $b^2r_{\new}\eta_{\new}\lambda_{\new}^+ \leq 0.5\lambda^-$ (because $b\leq0.1$, this will be satisfied if $r_{\new}\eta_{\new}\lambda_{\new}^+ \leq 50\lambda^-$); ?? may or may not need this
\label{xmin_cond}


\item model on $\wt$: Model \ref{wt_model} holds with $\epsilon_w^2 \le 0.03\zeta  \lambda^-$ % %\ref{wt_model_cor} holds with
\label{wt_cond}

\item independence: Let $\T:=\{\T_{\tilde{t}}\}_{\tilde{t}=1,2,\dots,t_{\max}}$. Assume that $\T,  \bm{w}_1, \bm{w}_2, \dots, \bm{w}_{t_{\max}}, \bnu_1, \bnu_2, \dots, \bnu_{t_{\max}}$ are mutually independent random variables.

\end{enumerate}
Then, with probability  $\ge 1 - 3n^{-10}$, at all times $t$,
\ben
\item $\T_t$ is exactly recovered, i.e. $\hat{\T}_t = \T_t$ for all $t$;

\item $\|\xt - \xhatt\|_2 \leq 1.34 \left(2\sqrt{\zeta} +  \sqrt{r_\new}\gamma_{\rmnew}  + \epsilon_w  \right)$ and $\|\lhat_t - \lt \|_2 \le \|\xt - \xhatt\|_2 + \epsilon_w$;

\item the subspace error $\SE_t := \|( \I - \hat{\bm{P}}_t \hat{\bm{P}}_t{}' ) \Pt \|_2 \le 10^{-2} \sqrt{\zeta}$ for all $t\in[t_{j}+d,t_{j+1})$;

\item the subspace change time estimates given by Algorithm \ref{reprocsdet} satisfy $t_j \leq \hat{t}_j \leq t_j + 2\alpha$;

\item its estimates of the number of new directions are correct: $\hat{r}_{j,\new,k} = r_{j,\new}$ for $j=1,\dots,J$; % and $k = 1,\dots,K$.

\item  eigenvalue clusters are recovered exactly: $\hat{\mathcal{G}}_{j,k} = \mathcal{G}_{j,k}$ for all $j$ and $k$; thus its estimate of the number of deleted directions is also correct.
    %$\hat{r}_j = \sum_{k=1}^{\vartheta_j} |\hat{\mathcal{G}}_{j,k}|$ and $\hat{r}_{j,\old} =
    %($\hat{r}_{j,old} = \hat{r}_{j-1} - \sum_{k=1}^{\vartheta_j} |\hat{\mathcal{G}}_{j,k}|$ and $\hat{r}_{j} =\hat{r}_{j,\new}+\sum_{k=1}^{\vartheta_j} |\hat{\mathcal{G}}_{j,k}|$)
\een
\end{theorem}


{\em Proof: } The proof outline is given in Section \ref{outline}. The proof is given in Sections \ref{pf_thm1_cor}, \ref{3_pfs}, \ref{3_pfs_del}.


\begin{remark}
Notice that the lower bound $|\mathcal{G}_{j,k}| \ge 0.15 (r+r_\new) $ can hold only if the number of clusters $\vartheta_j$ is at most 6. This is one choice that works along with the given bounds on other quantities such as $\rho^2 \beta$. It can be made larger if we assume a tighter bound on $\rho^2 \beta$ for example. But what will remain true is that our result requires the number of clusters to be $\bigo(1)$.
\end{remark}

\begin{remark} The independence assumption can again be replaced by the weaker one of Remark \ref{wt_model_weaker}.  \end{remark}

The extra assumption needed by the above result compared to Theorem \ref{thm1_cor_nodel} is the clustering one. Using this, ReProCS-cPCA is able to correctly estimate the current subspace. Thus,for $t \in [t_j, \that_j+\alpha]$, $\Phat_{t-1}$ is an accurate estimate of $\Span(\P_{t_j-1})$ where as when using ReProCS (and Theorem \ref{thm1_cor_nodel}), it is an estimate of $\Span([\P_0, \P_{t_1,\new}, \P_{t_2,\new}, \dots \P_{t_{j-1},\new}])$. Because of this, (i) the above result needs a much weaker denseness assumption, (ii) it does not need a bound on $J$, and (iii) it requires the new directions to only be orthogonal to $\Span(\P_{t_j-1})$.% (and not to $\Span([\P_0, \P_{t_1,\new}, \P_{t_2,\new}, \dots \P_{t_{j-1},\new}])$).
We discuss the results in detail in Sec. \ref{discussion}.


\begin{corollary} \label{thm1_cor_corol}
The following conclusions also hold under the assumptions of Theorem \ref{thm1_cor} with probability at least $1 - 3n^{-10}$.
\begin{enumerate}
%\item The estimates of the subspace change times given by Algorithm \ref{reprocsdet} satisfy $t_j \leq \hat{t}_j \leq t_j + 2\alpha$, for $j = 1,\dots, J$;
%\item The estimates of the number of new directions are correct, i.e. $\hat{r}_{j,\new,k} = r_{j,\new}$ for $j=1,\dots,J$ and $k = 1,\dots,K$;
\item The recovery error satisfies $\|\lhat_t - \lt \|_2 \leq \|\xt - \xhatt\|_2 + \epsilon_w$ and
\begin{align*}
\|\xt - \xhatt\|_2 \le
\begin{cases}
1.34 \left(2\sqrt{\zeta} +  \sqrt{r_{\new}}\gamma_{\rmnew} + \epsilon_w \right) & t \in \left[t_j, \that_j + \alpha \right] \\
1.34 \left(2.15\sqrt{\zeta} +  0.19\cdot(0.1)^{k-1}\sqrt{r_{\new}}\gamma_{\rmnew} + \epsilon_w \right) &   t \in \left[ \that_j+(k-1)\alpha + 1,  \that_j + k\alpha\right], \ k=2,3, \dots, K \\
2.67(\sqrt{\zeta} + \epsilon_w) & t \in \left[\that_j + K \alpha + 1,  \hat{t}_j + K \alpha + (\vartheta+1)\alpha \right] \\
2.67(\frac{r}{r+r_\new}\sqrt{\zeta} + \epsilon_w) & t \in \left[\that_j + K \alpha + (\vartheta+1)\alpha + 1, t_{j+1} - 1\right];
\end{cases}
\end{align*}
\item The subspace error satisfies,
\begin{align*}
\SE_t \leq
\begin{cases}
1  & t \in \left[t_j,\that_j + \alpha \right] \\
10^{-2} \sqrt{\zeta} +  0.19\cdot0.1^{k-1} & t \in \left[\that_j+(k-1)\alpha + 1,  \that_j + k\alpha \right], \ k=2,3, \dots, K  \\
10^{-2} \sqrt{\zeta}   &  t \in \left[\that_j + K \alpha + 1,  \hat{t}_j + K \alpha + (\vartheta+1)\alpha \right] \\
10^{-2} \frac{r}{r+r_\new}\sqrt{\zeta}   &  t \in \left[\that_j + K \alpha + (\vartheta+1)\alpha + 1, t_{j+1} - 1\right];
\end{cases}
\end{align*}
\end{enumerate}
\end{corollary}

%?? add the detailed bounds.


%?? move to Fact \ref{ltbnds}: From Model \ref{cor_model}, clearly $\|\lt\|_2 \le \frac{\sqrt{r}\gamma}{1-b}$. Moreover, $\lt$ can be expanded as follows.


{\bf Online matrix completion (MC). }
MC can be interpreted as a special case of RPCA and hence the same is true for online MC and online RPCA \cite{rpca,rrpcp_isit15}. In \cite{rrpcp_isit15}, we explicitly stated results for both. In a similar fashion, an analog of either of the above results can also be obtained for online MC.
%\end{remark}


{\bf Offline RPCA. }
In certain applications such as video analytics, an improved offline estimate of both the background and the foreground is desirable. In some other applications, there is no real need for an online solution. We show here that, with a delay of at most $(K+2)\alpha$ frames, by using essentially the same ReProCS algorithm with one extra step, it is possible to recover $\xt$ and $\lt$ with close to zero error.
\begin{corollary}[Offline RPCA]
Consider the estimates given in the last two lines of Algorithm \ref{reprocsdet}.
Under the assumptions of Theorem \ref{thm1_cor}, with probability at least $1 - 3n^{-10}$, at all times $t$,
$
\|\xt - \xhatt^{\mathrm{offline}}\|_2
%\le 1.2 (r+r_\new)\zeta (\sqrt{r}\gamma + \epsilon_w)
\le %1.2\sqrt{\zeta}(1+0.01 \epsilon_w)
2.67 (\sqrt{\zeta} +  \epsilon_w)
$, $\|\lhat_t^{\mathrm{offline}} - \lt \|_2 \le 2.67 (\sqrt{\zeta} +  2\epsilon_w)$,
and all its other conclusions hold.% (i.e. the support $\T_t$ is exactly recovered at all times and subspace error decays to a small value within a delay of at most $d$ frames after a subspace change);
\end{corollary}

Observe that the offline recovery error can be made smaller and smaller by reducing $\zeta$ (this, in turn, will result in an increased delay between subspace change times).
%
As can be seen from the last two lines of Algorithm \ref{reprocsdet}, the offline estimates are obtained at $t=\that_j+K \alpha$. Since $\that_j \le t_j+2 \alpha$, this means that the offline estimates are obtained after a delay of at most $(K+2)\alpha$ frames.



%{\bf Lower bound on outlier magnitudes. }
%The bound on $\sqrt{r_\new} \gamma_\new$ in condition \ref{xmin_cond} of Theorem \ref{thm1_cor} can be interpreted either as another ``slow subspace change" condition or as a lower bound on the minimum outlier magnitude. Since $\wt$ incorporates the small corruptions, the lower bound on outlier magnitudes makes sense. To understand this better, consider the case studied in \cite{rrpcp_icassp15,rrpcp_isit15}: $\mt = \lt + \xt$. Using Theorem \ref{thm1_cor}, we can get the following corollary for this case.
%
%\begin{corollary}[Corollary for the $\mt=\lt+\xt$ case]  %No lower bound on outlier magnitude
%Assume that $\mt = \lt + \xt$ for $t>t_\train$.
%
%For a $q>0$, let $\bm{x}_{t,\text{small}}(q)$ be a vector of entries of $\xt$ whose magnitude is smaller than $q$. Define  $\epsilon_w(q): = \max_t \|\bm{x}_{t,\text{small}}(q)\|_2$. Suppose that $\xt$ and $\lt$ are mutually independent; $\xt$'s are mutually independent; and there exists an $x_{\min}>0$ so that
%\bi
%\item $x_{\min} > 14 \epsilon_w (x_{\min}) + 14 ( \sqrt{r_\new}\gamma_{\new} + (\sqrt{r} + \sqrt{r_\new})\sqrt{\zeta} )$;  and $\| \bm{x}_{t,\text{small}}(x_{\min})\|_2^2 \le 0.03\zeta  \lammin$.
%\ei
%If the above assumption replaces condition \ref{wt_cond} and the condition ``$14 \xi \le \min_{t} \min_{i \in \T_t} |(x_t)_i|$" (in condition \ref{xmin_cond}) from Theorem \ref{thm1_cor}; and if all its other conditions hold with $\epsilon_w$ replaced by $\epsilon_w (x_{\min})$ and with $\T_t$ replaced by the set of indices of $\xt$ whose entries have magnitude equal to or larger than $x_{\min}$; then all its conclusions hold.
%\end{corollary}
%%\begin{proof} The proof is immediate and follows by letting $\wt \equiv \bm{x}_{t,\text{small}}(x_{\min})$. Notice that $\lt$ and $\xt$ mutually independent ensures that $\E[\lt \wt' | \T_t ] = 0$. This is true because $\lt$ and $\xt$ mutually independent implies that $\lt$ and $\wt$ are mutually independent and also that $\lt$ and $\T_t$ are mutually independent. As a result, conditioned on $\T_t$, $\lt$ and $\wt$ are mutually independent and so $\E[\lt \wt' | \T_t ] = 0$. \end{proof}
%
%


\subsection{Discussion} \label{discussion}
%Our result for online RPCA also needs a lower bound on $x_{\min}$ while PCP does not need this.
%Moreover, even with this, we can only guarantee very accurate recovery of $\lt$, while PCP guarantees exact recovery.
%compared to the PCP results \cite{rpca,rpca2,rpca_zhang} or the result from \cite{matcomp}  (or $\lt$ and $\xt$ in case or O-RPCA)

{\bf Online versus offline. }
We analyze an online algorithm that is faster and needs less storage. It needs to store only a few $n \times \alpha$ or $n \times r$ matrices, while  PCP needs to store matrices of size $n \times t_{\max}$.
%$\bigo(n t_{\max})$ since it needs to store the entire data matrix. thus the storage complexity is $\bigo(n \mathrm{polylog} n)$
%\Phat_{t,*}\Phat_{t,*}{}' - \Phat_{t,\new}\Phat_{t,\new}{}'
Other results for online algorithms include correctness results from \cite{rrpcp_icassp15,rrpcp_isit15} (discussed below), and partial results of Qiu et al. \cite{rrpcp_perf} and Feng et al. \cite{xu_nips2013_1}.
In \cite{xu_nips2013_1}, Feng et al. proposed a method for online RPCA and proved a partial result for their algorithm. Their approach was to reformulate the PCP program and to use this reformulation to develop a recursive algorithm that converged asymptotically to the solution of PCP as long as the basis estimate $\hat{\bm{P}}_t$ was full rank at each time $t$. Since this result assumed something about an intermediate algorithm estimate, $\hat{\bm{P}}_t$, it was  a {\em partial} result.
In \cite{rrpcp_perf}, Qiu et al. obtained a performance guarantee for ReProCS and ReProCS-cPCA that also needed intermediate algorithm estimates to satisfy certain properties. In particular, their result required that the basis vectors for the currently unestimated subspace, $\Span((I - \Phat_{t-1}\Phat_{t-1}{}')\P_{t_j,\new})$, be dense vectors. Thus, their result was also a  {\em partial} result.
In the current work, we remove this requirement and provide a {\em correctness result} for both ReProCS and ReProCS-cPCA. The assumption that helps us get this is Model \ref{sbyrho} on $\T_t$ (or its generalization given in Model \ref{general_model} later). Secondly, unlike \cite{rrpcp_perf}, we provide a correctness result for an automatic algorithm that does not assume knowledge of subspace change times, number of directions added or removed, or of the eigenvalue-based subspace clusters. Thirdly, we allow the $\lt$'s to follow an AR model where as \cite{rrpcp_perf} required independence over time.

To our knowledge, our work and \cite{rrpcp_icassp15,rrpcp_isit15} are the only correctness results for an online RPCA method. %All other results are either correctness results for batch techniques (not discussed here except PCP) or are partial results for online RPCA (discussed above).
Our work significantly improves upon the results of \cite{rrpcp_icassp15,rrpcp_isit15}. We allow the $\lt$'s to be correlated over time and use a first order AR model to model the correlation. As discussed earlier, this is significantly more practically valid than the independence assumption used in \cite{rrpcp_icassp15,rrpcp_isit15}. It includes independence as a special case. Moreover, with the extra clustering assumption, we are able to analyze Automatic ReProCS-cPCA in Theorem \ref{thm1_cor}. It needs a much weaker rank-sparsity assumption than what is needed by the result of \cite{rrpcp_isit15}, and it does not need a bound on $J$. % and it requires the new directions to only be orthogonal to $\Span(\P_{t_j-1})$.
We discuss this below.
%The earlier work \cite{rrpcp_icassp15,rrpcp_isit15} assumes that the $\lt$'s are mutually independent over time. This models static backgrounds in which the changes with respect to a mean background image are due to independent variations at each time, e.g., light flickers. However, in practice, background sequences often also change due to factors that are correlated over time, e.g., lake waters' motion. This can be better modeled using an autoregressive (AR) model. This is what is assumed in this work. We prove that as long as the AR coefficient is not too large, all the conclusions remain the same. The only change is in the setting of the algorithm parameters which now need to be larger. %The results for PCP \cite{rpca,rpca2,rpca_zhang} did not assume any model on the $\lt$'s at all.


%is $s \in \bigo(\frac{n}{(\log n)^8})$, $J \in \bigo(n)$, $r_\new \in \bigo(1)$ and $r \in \bigo(\log n)$. This means that \le r + J r_\new
{\bf Bounds on rank and sparsity. }
Let $\L:=[\ell_1, \ell_2 \dots \ell_{t_{\max}}]$, $\S:=[x_1, x_2 \dots x_{t_{\max}}]$, $r_{\text{mat}}:=\rank(\L)$ and let $s_{\text{mat}}$ be the number of nonzero entries in $\S$. With our models, $s_{\text{mat}} \le s t_{\max}$ and $r_{\text{mat}} \le r_0 + J r_\new$ with both bounds being tight. Models \ref{sbyrho} and \ref{dense_model} constrain $s$ and $s,r,r_\new$ respectively. Model \ref{sbyrho} needs $s \le \rho_2 n /\alpha$ and Model \ref{dense_model} needs $r s \in \bigo(n)$ and $r_\new s \in \bigo(n)$.
Using the expression for $\alpha$, it is easy to see that if $J \in \bigo(n)$, $r_\new \in \bigo(1)$ and $r \in \bigo(\log n)$, then
$\frac{1}{\alpha} \in \bigo(\frac{\zeta^2}{r^2 \log n}) = \bigo(\frac{1}{(\log n)^9})$
Alternatively, if $r \in \bigo(1)$, then $\frac{1}{\alpha} \in \bigo(\frac{1}{\log n})$.
%%$\alpha$ needs to be $\bigo(\frac{r^2 \log n}{\zeta^2}) = \bigo((\log n)^9)$ or larger. %$\alpha$ needs to be $\bigo(\log n)$ or larger. Suppose that $\alpha$ is set to its lower bound.
Thus, Theorem \ref{thm1_cor} definitely holds in two regimes of interest. The first is $J \in \bigo(n)$, $r_\new \in \bigo(1)$, $r \in \bigo(\log n)$, $s_{\text{mat}} \in \bigo(\frac{n t_{\max}}{(\log n)^9})$ and $r_{\text{mat}} \in \bigo(n)$.  The second is $J \in \bigo(n)$, $r_\new \in \bigo(1)$, $r \in \bigo(1)$, $s_{\text{mat}} \in \bigo(\frac{n t_{\max}}{\log n})$ and $r_{\text{mat}} \in \bigo(n)$. The second regime is more favorable when comparing bounds on $s_{\text{mat}}$ and $r_{\text{mat}}$, but, it also implies that the dimension of the subspace at any given time is $\bigo(1)$. This can be restrictive. The first regime allows the subspace dimension at any time to be $\bigo(\log n)$ which is more reasonable, but, because of this, it needs a tighter bound on $s$ and hence on $s_{\text{mat}}$.

In either regime, our requirements are weaker than those of the PCP results from \cite{rpca2,rpca_zhang}: they need $r_{\text{mat}} s = \bigo(n)$ which implies  $r_{\text{mat}} s_{\text{mat}} \in \bigo(n t_{\max})$; thus if $s_{\text{mat}} \in \bigo(\frac{n t_{\max}}{\log n})$, they would require $r_{\text{mat}}$ to be $\bigo(\log n)$. In the first regime, our conditions are slightly stronger than those of the PCP result from \cite{rpca} while in the second, they are comparable: \cite{rpca} needs $r_{\text{mat}} \in \bigo (\frac{n}{(\log n)^2})$ and $s_{\text{mat}} \in \bigo(n t_{\max})$.
%while the PCP results from \cite{rpca2,rpca_zhang} need a much stronger condition: t

Either set of requirements for Theorem \ref{thm1_cor} is significantly weaker than what is needed by Theorem \ref{thm1_cor_nodel} or by the results of \cite{rrpcp_icassp15,rrpcp_isit15}: both need $r_{\text{mat}} \in \bigo(\log n)$. This is because both analyze ReProCS without the cluster PCA based subspace deletion step. Suppose that $r_{j,\new}=r_\new$ for each $j$. For ReProCS without cluster PCA, this means that the dimension of the estimated subspace grows by $r_\new$ with each subspace change time. Thus, the maximum dimension of the estimated subspace is $r_{\text{mat}} = r_0 + J r_\new$ and this is what was used in place of $r$ in the denseness assumption as well in the bound on $\zeta$. This is why these results need $r_{\text{mat}}$ to be $\bigo(\log n)$. However, in Theorem \ref{thm1_cor}, we analyze ReProCS with cluster PCA. Cluster PCA is used to re-estimate the current subspace and thus effectively delete the subspace corresponding to the old directions. This ensures that the rank of the estimated subspace is also bounded by the rank of the true subspace at any time, i.e. by $r$. Thus, Theorem \ref{thm1_cor} only needs $r \in \bigo(\log n)$ while $r_{\text{mat}}$ can as large as $\bigo(n)$.

{\bf No bound on the number of subspace changes, $J$. }
%Another important advantage of the current result is as follows.
Notice that the result for ReProCS-cPCA given in Theorem \ref{thm1_cor} does not require an upper bound on the number of subspace changes, $J$. On the other hand, the results for ReProCS (both Theorem \ref{thm1_cor_nodel} and the results from \cite{rrpcp_icassp15,rrpcp_isit15}) require a bound on $J$ that is imposed by the denseness assumption: they need $(r_0 + J r_\new) 2s \mu \le 0.09 n$. All results for PCP need a bound on $r_{\mathrm{mat}}$. Under our model of subspace change, $r_{\mathrm{mat}}$ is at most $r_0+J r_\new$ with the bound being tight and hence the PCP results also need a bound on $J$. Of course, even for Theorem \ref{thm1_cor}, $J$ does affect bounds on other quantities: the result needs $t_{j+1}-t_j > d > K \alpha + (\vartheta+3) \alpha$ where $\alpha$ is an algorithm parameter that depends linearly on $\log J$. Thus, for any given value of $J$, the delay between subspace change times, $t_{j+1}-t_j$, and the duration for which the eigenvalues along the new directions need to be small (quantified in \eqref{anew_small}), $d$, need to grow as $\log J$.% the delay between subspace change times needs to satisfy

%The result holds as long as


%??? Mention : no bound on $J$ needed.
%
%The same thing is true for Corollary \ref{thm1_cor_corol} given here.
 %than what we now need: we only need $r \in \bigo(\log n)$ but $r_{mat}$ can be $\bigo(n)$. The reason is as follows. Suppose that $r_{j,\new}=r_\new$ for each $j$. For our older work, this meant that the dimension of the estimated subspace grew by $r_\new$ with each subspace change time. Thus, the maximum estimated subspace dimension was equal to $r_{mat} = r_0 + J r_\new$ and this is what was used in place of $r$ in the denseness assumption (Model \ref{dense_model}) as well in the bound on $\zeta$. This, in turn, meant that $r_{mat}$ needed to be $\bigo(\log n)$ with the same assumption on $s_{mat}$. However, in Theorems \ref{thm1} and \ref{thm1_cor}, the cluster PCA algorithm is used to re-estimate the current subspace and thus effectively delete the subspace corresponding to the old directions. This ensures that the rank of the estimated subspace is also bounded by the rank of the true subspace at any time, i.e. by $r$. %Thus, $r$ (which is the upper bound on the rank of the true subspace) gets used in our denseness assumption instead of $r_{mat}$. Thus only $r$ needs to be at most $\bigo(\log n)$ while $r_{mat}$ can as large as $\bigo(n)$.

%Models \ref{sbyrho} and \ref{dense_model} constrain $s$ and $s,r,r_\new, J$ respectively. Using the expression for $\alpha$, it is easy to see that $\alpha \in \bigo(\log n)$ as long as $J \in \bigo(n)$ and $r_\new = \bigo(1)$.  Thus, both conditions will hold if $s \in \bigo(\frac{n}{\log n})$, $r \in \bigo(\log n)$, $J \in \bigo(n)$ and $r_\new \in \bigo(\min(\log n,1)) = \bigo(1)$. Let $r_{\text{mat}}:=\rank(\L)$. Clearly $r_{\text{mat}} \le r_0 + J r_\new$. Let $s_{\text{mat}}:= t_{\max} s$ be a bound on the support size of $\S$. In terms of $r_{\text{mat}}$ and $s_{\text{mat}}$, what we need is $r_{\text{mat}} \in \bigo(n)$ and $s_{\text{mat}} \in \bigo(\frac{n t_{\max}}{\log n})$.  This is similar to what the PCP result from \cite{rpca} needs ($r_{\text{mat}} \in \bigo (\frac{n}{(\log n)^2})$, $s_{\text{mat}} \in \bigo(n t_{\max})$) and significantly weaker than what the PCP results from \cite{rpca2,rpca_zhang} need. This is also significantly weaker than what the results from \cite{rrpcp_icassp15,rrpcp_icassp15,rrpcp_isit15_arxiv} need: they need $r_{\text{mat}} \in \bigo(\log n)$.

{\bf Assumptions on how often the outlier support $\T_t$ needs to change. }
An important advantage of our work over PCP and other batch methods is that we allow more correlated changes of the set of outliers over time. From the assumption on $\T_t$, it is easy to see that we allow the number of outliers per row of $\L$ to be $\bigo(t_{\max})$, as long as the sets follow Model \ref{sbyrho}\footnote{In a period of length $\alpha$, the set $\T_t$ can occupy index $i$ for at most $\rrho\beta$ time instants, and this pattern is allowed to repeat every $\alpha$ time instants. So an index can be in the support for a total of $\rrho\beta\frac{t_{\max}}{\alpha}$ time instants and the model assumes $\rrho \beta \le \frac{0.0001 \alpha}{\rrho}$ for a constant $\rrho$. Thus an index $i$ can be part of the support $\T_t$ for at most $\frac{0.0001}{\rho} t_{\max} \in \bigo(t_{\max})$ time instants.}. %\footnote{If we split $t_{\max}$ into intervals of length $\alpha$, then the bound on $s$ ensures that an index is not re-visited; the bound on $\beta$ ensures that we need the support to change at least once every $0.0001 \alpha$ frames; also because object moves by s/rho and never comes back, it means a given index remains in the support for at most rho C alpha frames; this pattern can repeat again and so the maximum number of times for which an index could be in the support is C tmax.   as long as they follow the model}
This is the same as what our previous results \cite{rrpcp_icassp15,rrpcp_isit15} also allowed.
On the other hand, the PCP results from \cite{rpca2,rpca_zhang} need this number to be $\bigo(\frac{t_{\max}}{r_{\text{mat}}})$ which is stronger. %than what we need.
The PCP result from \cite{rpca} needs that the set $\cup_{t=1}^{t_{\max}} \T_t$ should be generated uniformly at random which is even stronger. %However their result does not impose any bound on $|\T_t|$ at a given time $t$, while we require $|\T_t| \le s \in \big(\frac{n}{\mathrm{polylog}(n)})$. This bound is similar to or weaker than what the PCP results from \cite{rpca2,rpca_zhang} need: they need $s r_{mat} = \bigo(n)$.

%We should note though that our result needs a bound on $\T_t$ at each time $t$ where as the results for PCP do not need such a bo


%these sets to be independent
%It needs to store only a few $n \times \alpha$ or $n \times r_{\text{mat}}$ matrices, thus the storage complexity is $\bigo(n \log n)$ while that for PCP is $\bigo(n t_{\max})$.

%Moreover, we do not need any assumption on the right singular vectors of $\L$ while all results for PCP do. Finally, we analyze an {\em online} algorithm that is faster and needs less storage.



{\bf Other assumptions. } %Assumptions on subspace change. } %Assumptions on left and right singular vectors of $\L$. }  on the subspace change of the $\lt$'s and on the clustering of the eigenvalues
The above advantages are obtained because we use extra assumptions on $\lt$. We assume (i) accurate knowledge of the initial subspace (or available outlier free data from which this can be obtained), (ii) slow subspace change as quantified by \eqref{anew_small} and the lower bound on the delay between subspace change times, and (iii) for a period of time after the previous subspace change has stabilized, we assume that the eigenvalues along the various subspace directions can be clustered into a few clusters. The result of \cite{rrpcp_isit15} required (i) and (ii) but not (iii). On the other hand, the PCP results \cite{rpca,rpca2,rpca_zhang} do not need any of the above. But they need other extra assumptions. They require denseness of the right singular vectors of $\L$ and a bound on the maximum absolute entry of the matrix $U V'$ where $U$ is the matrix of left singular vectors of $\L$ and $V$ is the matrix of its right singular vectors. In our notation $\Span(U) = \Span([P_0, P_{1,\new}, \dots P_{J,\new}])$. We assume denseness of $U$ but not of the right singular vectors.
%The bound on the maximum absolute entry of $U V'$ can be related to our assumed bounds on $\gamma$ and $\gamma_\new$. %To understand this, suppose that $\Lamt=\sigma^2 \I$ for all t. Then $UV' = \L$ and then the bound on its maximum absolute entry is the same as the bound on $\gamma$. The clusters are defined as sets of eigenvalues with a small enough condition number (below $g^+$) and we require that the smallest eigenvalue of the $k$-th cluster be much larger than the largest eigenvalue of the $(k+1)$-th cluster.

{\bf Setting algorithm parameters. }
Our result needs five algorithm parameters to be appropriately set. Some of these require knowing at least an upper bound on the model parameters. Our result needs to know upper bounds on $\gamma, \gamma_\new$, $r_0, r, r_\new$, $b$, and $g^+$. The PCP results need this for none \cite{rpca} or at most one \cite{rpca2,rpca_zhang} algorithm parameter.
We briefly explain in Sec. \ref{param_set} how to set algorithm parameters automatically for practical experiments.
%Moreover, the actual values used for these parameters in practical experiments are much smaller.


{\bf Other work. }
A recent work that uses knowledge of the initial subspace estimate but performs recovery in a piecewise batch fashion is modified-PCP \cite{zhan_pcp}. Like PCP, the result for modified PCP also needs uniformly randomly generated support sets which is stronger than what we need. But, like PCP, it does not need the other extra assumptions that ReProCS needs. Another somewhat related work is the algorithm and correctness result of Feng et al. \cite{xu_nips2013_2} on online PCA with contaminated data. This does not model the outlier as a sparse vector but defines anything that is far from the data subspace as an outlier. %The theorems in both papers only talk about asymptotically converging to the solution of the batch problem. %, whereas in the current work, we exploit slow subspace change to actually relax a key assumption needed by the batch methods (that of uniformly distributed random supports or of very frequent support change).  (so the above comparisons still apply)



%Its assumption on the rank-sparsity product is weaker than that of PCP, and hence weaker than that needed by this work.
%A detailed simulation comparison between modified-PCP, ReProCS and PCP demonstrating both these things is available in \cite[Fig. 6]{zhan_pcp}.

%detects subspace change automatically and also estimates the rank of the new subspace automatically.

%
%{\bf Other assumptions. }
%%  on subspace change of the $\lt$'s
%We get the above advantages over PCP because we use extra assumptions - accurate initial subspace knowledge, slow subspace change and and clustered eigenvalues after a subspace change has stabilized. Also our result needs five algorithm parameters to be appropriately set. The actual values used for these parameters in experiments is much smaller than what our theorem requires. The PCP results need this for none \cite{rpca} or at most one \cite{rpca2,rpca_zhang} algorithm parameter.
%



\begin{algorithm}[t!] %$\Phat_{t_\train}$, $\lamtrain$,
%\caption{Automatic Online/Offline Add-Delete ReProCS (Auto-On/Off-AddDel-ReP)}\label{reprocsdet}
\caption{Automatic ReProCS-cPCA}\label{reprocsdet}
{\bf Parameters}: $\alpha$, $K$, $\xi$, $\omega$, $\ghatp$, \ {\bf Inputs}: $\bm{m}_t$ for each $t$, \ {\bf Output}: $\xhatt$, $\lhatt$,  $\Phat_{t}$, $\that_{\jhat}$, $\hat{r}_{\jhat,\new,k}$, $\hat{G}_{j,k}$

Compute $\lamtrain$ as the $r_0$-th eigenvalue of $\frac{1}{t_\train} \sum_{t=1}^{t_\train} \mt \mt'$ and $\Phat_{t_\train}$ as its top $r_0$ eigenvectors.%\leftarrow \mathrm{eigenvectors}(\frac{1}{t_\train} \sum_{t=1}^{t_\train} \mt \mt',,r_0)$
%$ as the $r_0$ top left singular vectors of this matrix.

Set $\thresh=\frac{\lamtrain}{2}$. %(this is the eigenvalue threshold that will be used to detect subspace change).
%
Set $\Phat_{t,*} \leftarrow \Phat_{t_\train}$, $\Phat_{t,\new} \leftarrow [.]$, $\jhat \leftarrow 0$,  $\mathrm{phase} \leftarrow \mathrm{detect}$.

For every $t > t_\train$, do
\ben

\item {\bf Estimate $\T_t$ and $\xt$: }
\ben
\item \label{othoproj} compute $\bm{\Phi}_{t} \leftarrow \bm{I} - \Phat_{t-1} \Phat_{t-1}{}'$ and $\bm{y}_t \leftarrow \bm{\Phi}_{t} \bm{m}_t$

\item \label{Shatcs} solve $\min_{\bm{x}} \|\bm{x}\|_1 \ s.t. \ \|\bm{y}_t - \bm{\Phi}_{t} \bm{x}\|_2 \leq \xi$ and let $\hat{\bm{x}}_{t,\cs}$ denote its solution
\item \label{That} compute $\hat{\mathcal{T}}_t = \{i: \ |(\hat{\bm{x}}_{t,\cs})_i| > \omega\}$
\item \label{LS} LS: compute $\hat{\bm{x}}_t= \I_{\hat{\mathcal{T}}_t} ((\bm{\Phi}_t)_{\hat{\mathcal{T}}_t})^{\dag} \bm{y}_t$
\een

\item {\bf Estimate $\bm{\ell}_t$: }
$\hat{\bm{\ell}}_t \leftarrow \bm{m}_t - \hat{\bm{x}}_t $ %where $\bm{\Phi}_t:= I - \Phat_{t-1} \Phat_{t-1}{}'$

\item {\bf Subspace Update: }

If $t \mod \alpha \neq 0$ then $\Phat_{t,*} \leftarrow \Phat_{t-1,*}$, $\Phat_{t,\new} \leftarrow \Phat_{t-1,\new}$, $\Phat_{t} \leftarrow [\Phat_{t,*} \ \Phat_{t,\new}]$

 If $t \mod \alpha = 0$  then %{\em detection or projection PCA or cluster PCA}
\\
{\bf if  $\mathrm{phase} = \mathrm{detect}$ then}
\begin{enumerate}

\item \label{detect} Set $ u = \frac{t}{\alpha}$ and compute $\bm{\mathcal{D}}_u = (\I - \Phat_{u\alpha-1,*} \Phat_{u\alpha-1,*}{}') [\lhat_{(u-1)\alpha+1}, \dots \lhat_{u\alpha}]$

\item $\Phat_{t,*} \leftarrow \Phat_{t-1,*}$, $\Phat_{t,\new} \leftarrow \Phat_{t-1,\new}$, $\Phat_{t} \leftarrow [\Phat_{t,*} \ \Phat_{t,\new}]$ %$\Phat_{t} \leftarrow \Phat_{t-1}$

\item \label{change} If $\lambda_{\max} (\frac{1}{\alpha} \bm{\mathcal{D}}_u \bm{\mathcal{D}}_u{}'  ) \ge \thresh$  then
\begin{enumerate}
\item $\mathrm{phase} \leftarrow \mathrm{pPCA}$, $\jhat \leftarrow \jhat+1$, $k \leftarrow 0$, $\that_{\jhat} = t$
%\item {\bf cluster PCA -- Algorithm \ref{cPCA_algo}.}
\end{enumerate}

\end{enumerate}
%
{\bf else if $\mathrm{phase} = \mathrm{pPCA}$ then}
%
\begin{enumerate}
\item Set $ u = \frac{t}{\alpha}$ and compute
$\bm{\mathcal{D}}_u = (\I - \Phat_{u\alpha-1,*} \Phat_{u\alpha-1,*}{}') [\lhat_{(u-1)\alpha+1}, \dots \lhat_{u\alpha}]$

\item\label{PCA} $\Phat_{t,\new} \leftarrow \text{eigenvectors}\left(\frac{1}{\alpha} \bm{\mathcal{D}}_u \bm{\mathcal{D}}_u{}',\thresh\right)$,  $\Phat_{t,*} \leftarrow \Phat_{t-1,*}$, $\Phat_{t} \leftarrow [\Phat_{t,*} \ \Phat_{t,\new}]$

\item  $k \leftarrow k+1$, set $\hat{r}_{j,\new,k} = \rank(\Phat_{t,\new})$

\item If $k == K$, then
\ben \item $\mathrm{phase} \leftarrow \mathrm{cPCA}$,  reset $k \leftarrow 0$ \een % $\Phat_{t,\new} \leftarrow [.]$
%\begin{enumerate}
%\item $\mathrm{phase} \leftarrow \mathrm{cPCA}$
%\item reset $k \leftarrow 1$
%%\item $\Phat_{t,*} \leftarrow [\Phat_{t-1,*} \ \Phat_{t,\new}]$ \item $\Phat_{t} \leftarrow \Phat_{t,*}$
%\item $\Phat_{t,\new} \leftarrow [.]$
%\end{enumerate}
\end{enumerate}
{\bf else  if $\mathrm{phase} = \mathrm{cPCA}$ then}
\ben
\item cluster PCA (summarized in Algorithm \ref{clusterPCA}); %set $\Phat_{t} \leftarrow [\hat{\bm{G}}_{j,1} \cdots \hat{\bm{G}}_{j,\vartheta}]$
\item set $\Phat_{t,*} \leftarrow \Phat_{t}$, $\Phat_{t,\new}\leftarrow [.]$,
\item $\mathrm{phase} \leftarrow \mathrm{detect}$, reset $k \leftarrow 0$%, $\Phat_{t,\new} \leftarrow [.]$
\een
{\bf end-if}
\een
$\mathrm{eigenvectors}(\bm{\mathcal{M}},\thresh)$ returns a basis matrix for the span of eigenvectors with eigenvalue above $\thresh$.
$\mathrm{eigenvectors}(\bm{\mathcal{M}},,r)$ returns a basis matrix for the span of the top $r$ eigenvectors.% (eigenvectors with the largest $r$ eigenvalues).

{\bf Offline RPCA: } at $t = \that_j + K \alpha$, for all $t \in [\that_{j-1}+ K \alpha+1,  \that_j + K \alpha]$, compute
%\item Compute $\bm{\Phi}_{t_{\max}}:= \I - \Phat_{t_{\max}} \Phat_{t_{\max}}{}'$
\[
\xhatt^{\mathrm{offline}} \leftarrow \I_{\hat{\mathcal{T}}_t} ((\bm{\Phi}_{\that_j + K \alpha})_{\hat{\mathcal{T}}_t})^{\dag} \bm{\Phi}_{\that_j + K \alpha} \bm{m}_t
\text{  and  }
\lhatt^{\mathrm{offline}} \leftarrow \mt - \xt
\]
\end{algorithm}


\begin{algorithm}[t!]
\caption{\small{cluster PCA}}% (called from Algorithm \ref{reprocsdet})}}
\label{clusterPCA}
\ben

\item If $k==0$, estimate the clusters
\ben
\item Set $ u = \frac{t}{\alpha}$ and compute $\hat{\bm{\Sigma}}_{\mathrm{sample}} =  \frac{1}{\alpha}\sum_{t =(u-1)\alpha+1}^{u \alpha} \lhatt\lhatt{}'$. Let $\hat\lambda_i$ denote its $i$-th largest eigenvalue.

\item To get the first cluster $\hat{\mathcal{G}}_{j,1}$, we start with the index of the first (largest) eigenvalue and keep adding indices of the smaller eigenvalues to it until $\frac{\hat\lambda_1}{\hat\lambda_{i+1}} > \ghatp$ but $\frac{\hat\lambda_1}{\hat\lambda_{i}} \le \ghatp$ or until $\hat\lambda_{i+1} < 0.25 \lamtrain$. We set  $\hat{\mathcal{G}}_{j,1} = \{1,2, \dots i\}$.
%To compute the first cluster, $\hat{\mathcal{G}}_{j,1}$, start with $i=1$ and keep adding the indices of the next smaller eigenvalues until either the ratio of the maximum to the minimum eigenvalue first exceeds $\ghatp$ or the next eigenvalue is below $0.25 \lamtrain$. More precisely, set $\hat{\mathcal{G}}_{j,1} \leftarrow \{1,2,\dots i\}$ if the first (largest) eigenvalue and keep adding smaller eigenvalues to the set until either the ratio of the maximum to the minimum eigenvalue first exceeds $\ghatp$ or the next eigenvalue is below $0.25 \lamtrain$. Suppose this happens for the $(k_1+1)$-th eigenvalue. Then, define $\hat{\mathcal{G}}_{j,1} = \{1,2, \dots, k_1\}$.
\\
For  $\hat{\mathcal{G}}_{j,2}$, start with the $(i+1)$-th eigenvalue and repeat the above procedure.
Repeat the above for each new cluster and stop when there are no more eigenvalues larger than $0.25 \lamtrain$. %\footnotemark.

\item  $k \leftarrow k+1$, $\Phat_{t,*} \leftarrow \Phat_{t-1,*}$, $\Phat_{t,\new} \leftarrow \Phat_{t-1,\new}$, $\Phat_{t} \leftarrow [\Phat_{t,*} \ \Phat_{t,\new}]$
\een

\item If $1 \le k \le \vartheta$, estimate the $k$-th cluster's subspace by cluster PCA
\ben
\item Set $ u = \frac{t}{\alpha}$,  set $\hat{\bm{G}}_{j,0} \leftarrow [.]$. %For $i = 1,2,\dots, \hat{\vartheta}_{j}$, do
  \bi
  \item let $\hat{\bm{G}}_{j,\det,k}:= [\hat{\bm{G}}_{j,0},\hat{\bm{G}}_{j,1}, \dots \hat{\bm{G}}_{j,k-1}]$ and let $\bm\Psi_k:=(\I -\hat{\bm{G}}_{j,\det,k} \hat{\bm{G}}_{j,\det,k}{}')$ (notice that $\bm\Psi_{j,1}=\I$);  compute
  $\bm{\mathcal{M}}_{\mathrm{cpca}} = \bm\Psi_k \left(\frac{1}{\alpha}\sum_{t \in (u-1)\alpha+1}^{u \alpha} \lhat_t \lhat_t{}'\right) \bm\Psi_k$

  \item compute $\hat{\bm{G}}_{j,k} \leftarrow \mathrm{eigenvectors}(\bm{\mathcal{M}}_{\mathrm{cpca}},,|\hat{\mathcal{G}}_{j,k}|)$
%  top $|\hat{\mathcal{G}}_{j,k}|$ eigenvectors of $\bm{\mathcal{M}}_{\mathrm{cpca}}$
  \ei

\item $k \leftarrow k+1$, $\Phat_{t,*} \leftarrow \Phat_{t-1,*}$, $\Phat_{t,\new} \leftarrow \Phat_{t-1,\new}$, $\Phat_{t} \leftarrow [\Phat_{t,*} \ \Phat_{t,\new}]$
\een

\item If $k==\vartheta$, set $\Phat_{t} \leftarrow [\hat{\bm{G}}_{j,1} \cdots \hat{\bm{G}}_{j,\vartheta}]$.
%\bi
%\item set $\Phat_{t} \leftarrow [\hat{\bm{G}}_{j,1} \cdots \hat{\bm{G}}_{j,\vartheta}]$
%\ei

\een
\end{algorithm}


\section{Automatic ReProCS-cPCA} \label{algo_sec}

The automatic ReProCS-cPCA algorithm is summarized in Algorithm \ref{reprocsdet}. It proceeds as follows. It begins by estimating the initial subspace as the top $r_0$ left singular vectors of $[\bm{m}_1,\bm{m}_2,\dots, \bm{m}_{t_\train}]$. Let $\Phat_t$ denote the basis matrix for the subspace estimate at time $t$.
At time $t$, if the previous subspace estimate, $\Phat_{t-1}$, is accurate enough, because of the ``slow subspace change" assumption, projecting $\mt = \xt + \lt + \wt$ onto its orthogonal complement nullifies most of $\lt$. Specifically, we compute $\bm{y}_t:= \bm{\Phi}_t \mt$ where $\bm{\Phi}_t:= \I - \Phat_{t-1}\Phat_{t-1}{}'$. Clearly, $\bm{y}_t = \bm{\Phi}_t \xt + \bm{b}_t$ where $\bm{b}_t:= \bm{\Phi}_t\lt + \bm{\Phi}_t \wt$ and it can be argued that $\| \bm{b}_t \|_2$ is small: $\| \bm{\Phi}_t\lt\|_2$  is small due to the slow subspace change assumption and $\|\wt\|_2 \le \epsilon_w$.
Thus recovering $\xt$ from $\bm{y}_t$ becomes a traditional sparse recovery problem in small noise \cite{candes_rip}. We recover $\xt$ by $l_1$ minimization with the constraint $\| \bm{y}_t - \bm{\Phi}_t x\|_2 \le \xi$ and estimate its support by thresholding using a threshold $\omega$. We use the estimated support, $\That_t$, to get an improved debiased estimate of $\xt$, denoted $\xhatt$, by least squares (LS) estimation on $\That_t$. We then estimate $\lt$ as $\lhat_t = \mt - \xhatt$.
By the denseness assumption given in Model \ref{dense_model}, it can be argued that the restricted isometry constant (RIC) of $\bm{\Phi}_t$ will be small. Under the theorem's assumptions, we can bound it by 0.14. This ensures that a sparse $\xt$ is indeed accurately recoverable from $\bm{y}_t$.
%
%By the denseness assumption given in Model \ref{dense_model}, it can be argued that the restricted isometry constant (RIC) \cite{decodinglp} of $\bm{\Phi}_t$ will be small.
With the support estimation threshold $\omega$ set as in Theorem \ref{thm1_cor}, it can be argued that the support will be exactly recovered, i.e., $\That_t=\T_t$. Let $\et: = \lt - \lhat_t$.
With this, it is clear that $\et =  (\xhatt - \xt) - \wt$ satisfies
\bea
\et = \I_{\T_t} [(\bm{\Phi}_t)_{\T_t}{}'(\bm{\Phi}_t)_{\T_t}]^{-1} \I_{\T_t}{}' \bm{b}_t - \wt = \I_{\T_t} [(\bm{\Phi}_t)_{\T_t}{}'(\bm{\Phi}_t)_{\T_t}]^{-1} \I_{\T_t}{}' \bm{\Phi}_t (\lt+\wt) - \wt.
\label{etdef_0}
\eea
%where $\bm\Phi_t:=\I - \Phat_{t-1} \Phat_{t-1}{}'$.
% (see Lemma \ref{kappadelta})  (see Lemma \ref{cslem}) \I_{\T_t} (\bm{\Phi}_t)_{\T_t}{}^\dag \bm{b}_t  - \wt =
Using the bound on the RIC of $\bm\Phi_t$, clearly $\|(\bm{\Phi}_t)_{\T_t}{}'(\bm{\Phi}_t)_{\T_t}^{-1}\|_2 \le (1-0.14)^{-1} < 1.2$. Thus,  $\|\et\|_2 \le 1.2 \|\bm{b}_t\|_2 + \epsilon_w$, i.e., it is small too. In other words, $\lt$ is accurately recovered.  %, using the fact that $\|\wt\|_2$ is small, \|\bm{\Phi}_t\lt\|_2 + 2.2 \|\wt \|_2

The estimates $\lhatt$ are used in the subspace estimation step which involves (i) detecting subspace change; (ii) $K$ steps of projection-PCA, each done with a new set of $\alpha$ frames of $\lhatt$, to get an accurate enough estimate of the newly added subspace; and (iii) cluster PCA to delete the old subspace by re-estimating the current subspace. At the end of the projection PCA step, the estimated subspace dimension is at most $r+r_\new$, and after cluster PCA, it comes down to at most $r$.

{\em Subspace update. }
In the subspace update step, the algorithm switches between the ``detect" phase, the ``pPCA" phase and the ``cPCA" phase. It starts in the ``detect" phase. When a subspace change is detected, i.e. at $t= \that_j$, it enters the ``pPCA" phase. After $K$ iterations of projection-PCA, i.e. at $t=\that_j+K\alpha$, the new subspace has been accurately estimated. At this time, it enters the ``cPCA" phase. At $t=\that_j+K\alpha+ (\vartheta+1)\alpha$, cluster PCA is done. At this time, it enters the ``detect" phase again and remains in it until the next subspace change is detected.
%for $u=1,2,\dots,\llfloor\frac{t_{\max}}{\alpha}\rrfloor$
We detect the $j$-th subspace change as follows. Let $\Phat_* := \Phat_{\that_{j-1}+K\alpha+(\vartheta+1)\alpha}$. We detect change by comparing the eigenvalues of $\frac{1}{\alpha}\sum_{t} (\I-\hat{\bm{P}}_*\hat{\bm{P}}_*{}')\lhat_t \lhat_t' (\I-\hat{\bm{P}}_*\hat{\bm{P}}_*{}')$ to a chosen threshold at every $t=u\alpha$ when the algorithm is in the ``detect" phase.
% and suppose that the subspace $\Span(\bm{P}_{*})$ has been accurately recovered, i.e. we have $\Phat_*$ so that $\mathrm{dif}(\Phat_*, \bm{P}_*) \ll 1$
%In order to work properly, the algorithm first must not falsely detect new directions when none are present and it must detect subspace change within a short delay after it has occurred. The former will occur because, conditioned on accurate recovery of the current subspace, $M_u$ will be very small when no new directions are present. If the previous subspace were exactly recovered, this matrix would be zero. In our case, the recovery is only accurate and so we show that all eigenvalues of this matrix will be below the chosen threshold (see Lemma \ref{falsedet_del}).  Next consider detection of the subspace change after it has occurred. When $u = u_j:= \llceil \frac{t_j}{\alpha} \rrceil$, i.e. when $t_j$ is in the interval $\big[(u-1)\alpha+1,u\alpha\big]$, not all of the $\lt$'s in this interval will contain new directions. Thus, depending on where in the interval $t_j$ lies, the algorithm may or may not detect the subspace change. However, in the {\em next} interval, $[u_j\alpha+1,(u_j+1)\alpha]$, all of the $\lt$'s will contain new directions, and we can prove that the subspace change will be detected whp (see Lemma \ref{det}). Thus, whp, either $\hat{t}_j = u_j \alpha$, or $\hat{t}_j = (u_j+1)\alpha$. Thus, we will be able to show that $t_j \le \that_j \le t_j+2\alpha$ whp. ???


{\em Projection-PCA (p-PCA). }
We use projection-PCA to estimate the newly added subspace. The reason this cannot be done using standard PCA is as follows \cite{rrpcp_perf}. Let $\sum_t$ denote a sum over an $\alpha$ length time interval. %$t \in [\that_j+(k-1)\alpha+1, \that_j+k\alpha]$.
Because of how $\lt$ is recovered, the error, $\et$, in the estimate of $\lt$, $\lhat_t$, is correlated with $\lt$. This is evident from \eqref{etdef_0}. %Under the theorem assumptions, the dependence is, in fact, linear (see \eqref{etdef_0}).
Due to this, the dominant terms in the perturbation seen by standard PCA, $\frac{1}{\alpha} \sum_t \lhatt \lhatt{}' - \frac{1}{\alpha} \sum_t \lt {\lt}'$,
are $\frac{1}{\alpha} \sum_t \lt {\et}'$ and its transpose\footnote{When $\lt$ and $\et$ are uncorrelated and one of them is zero mean, it can be argued by law of large numbers that, whp, these two terms will be close to zero and $\frac{1}{\alpha} \sum_t \et {\et}'$ will be the dominant term. %Thus, if $\cov(\et)$ is small, then $\frac{1}{\alpha} \sum_t \et \et'$, and hence the perturbation, will be small too.
}.
Thus, when the condition number of $\cov(\lt)$ is large, it is not possible to argue that the perturbation will be small compared to the smallest eigenvalue of $\cov(\lt)$. With a large perturbation, either the $\sin \theta$ theorem \cite{davis_kahan} (that bounds the subspace error between the eigenvectors of the true and estimated sample covariance matrices) cannot be applied or it gives a very large and useless bound.

%\Phat_{t_j-1}$
Projection-PCA addresses the above issue as follows. Consider the $j$-th subspace change. %a $t \in [t_j, t_{j+1}-1]$.  , the $j$-th subspace change will get detected at a time $t$ that occurs after $t_j$ but not after $t_j + 2\alpha$, i.e.,
Let $\bm{P}_* := \P_{t_{j-1}}$, $\P_{\new}:=\P_{t_j,\new}$, and $\Phat_* := \Phat_{\that_{j-1}+K\alpha+(\vartheta+1)\alpha}$. %Suppose that the subspace $\Span(\bm{P}_{*})$ has been accurately recovered, i.e., $\mathrm{dif}(\Phat_*, \bm{P}_*) \le r \zeta \ll 1$. At a time at or after $t_j+\alpha$ if we project the $\alpha$ previous $\lhat_t$'s orthogonal to $\Span(\Phat_*)$, we will considerably reduce the perturbation seen by the PCA step. As explained above, we detect subspace change by checking if the maximum singular value of the matrix formed by these projected $\lhat_t$'s is above a threshold.
Denote the time at which this change is detected by $\that_j$. As explained in \cite{rrpcp_isit15}, it is easy to show that, whp, $t_j \le \that_j \le t_j+2\alpha$.
After $\that_j$ we use SVD on $K$ different sets of $\alpha$ frames of the $\lhat_t$'s projected orthogonal to $\Phat_*$ to get $K$ estimates of the new subspace $\Span(\bm{P}_{\new})$.
%(we can show that each new estimate improves upon the previous one).
We get the $k$-th estimate, $\Phat_{\new,k}$, as the left singular vectors of $(\I - \Phat_* \Phat_*{}')[\lhat_{\that_j+(k-1)\alpha+1}, \dots , \lhat_{\that_j+ k\alpha}]$ with singular values above a threshold. After each projection-PCA step, we update $\Phat_t$ as $\Phat_t = [\Phat_* \ \textit{} \Phat_{\new,k}]$. This ensures that the error $\et$ is smaller for the next projection-PCA interval compared to the previous one and hence the subspace estimates also improve with each iteration. The above is done $K$ times with $K$ chosen so that, by $t=\that_j+K\alpha$, the error in estimating the new subspace is below $r_\new \zeta$. This ensures that, at this time, $\SE_t \le r \zeta +r_\new\zeta$.
%the end of the $K$-th projection-PCA step, i.e.,
%Finally at $t = \that_j+K\alpha$, we update $\Phat_*$ as $[\Phat_{*} \ \Phat_{\new,K}]$.%

%space spanned by all the previously estimated eigenvectors  (reduce the error to $r \zeta$)
{\em Cluster PCA for deleting directions by re-estimating the subspace. } The next step is to delete the subspace $\Span(\P_{j,\old})$ from $\Phat_t$.  The goal of doing this is to reduce the subspace error from $(r+r_\new) \zeta$ to $r \zeta$. The simplest way to do this would be to re-estimate $\Span(P_t)$ by standard PCA, i.e. compute the eigenvectors of $\frac{1}{\alpha}\sum_{t = \that_j+K \alpha + 1}^{t = \that_j+K \alpha + \alpha} \lhat_t \lhat_t'$ with eigenvalues above a threshold. However, since $\lt$ and $\et$ are correlated, this will cause a problem similar to the one described above. It will work only if the condition number of $\cov(\lt)$ is small. This is impractical though since we assume that $\lt$ can be large but structured noise.
Hence we re-estimate the subspace by developing a generalization of the projection-PCA idea that we call {\em cluster PCA (cPCA)}. This relies on the clustering assumption given in Model \ref{clust_model}.

cPCA proceeds as follows. We first estimate the clusters as follows. We compute the empirical covariance matrix of $\lhatt$'s after the new subspace is accurately estimated: $\hat{\bm\Sigma}_{\mathrm{sample}} = \frac{1}{\alpha} \sum_{t=\that_j+K\alpha+1}^{t=\that_j+K\alpha+\alpha} \lhatt \lhatt'$ and obtain its EVD. Let $\hat\lambda_i$ denote its $i$-th largest eigenvalue.
To get the first cluster $\hat{\mathcal{G}}_{j,1}$, we start with the index of the first (largest) eigenvalue and keep adding indices of the smaller eigenvalues to it until $\frac{\hat\lambda_1}{\hat\lambda_{i+1}} > \ghatp$ but
$\frac{\hat\lambda_1}{\hat\lambda_{i}} \le \ghatp$ or until the next eigenvalue $\hat\lambda_{i+1} < 0.25 \lamtrain$. We set  $\hat{\mathcal{G}}_{j,1} = \{1,2, \dots i\}$.
To get the second cluster we repeat the same procedure but starting with the $(i+1)$-th eigenvalue. We repeat this until there is no eigenvalue larger than $0.25 \lamtrain$. Observe that $\ghatp$ is set to a value that is a little larger than $g^+$ (see Theorem \ref{thm1_cor}). This is needed to allow for the fact that $\hat\lambda_i$ is not equal to the $i$-th eigenvalue of $\Lamj$ but is within a small margin of it. For the same reason, we need to also use a ``zeroing" threshold of $0.25 \lamtrain$ (notice that $\hat{\bm\Sigma}_{\mathrm{sample}}$ is not exactly low rank). This, along with appropriately setting $\ghatp$, and with using the separation condition from Model \ref{clust_model} ensures that, whp, all the clusters are correctly recovered.

Let $\bm{G}_{j,k}:= (\P_j)_{\hat{\mathcal{G}}_{j,k}}$.
Next, we estimate the subspace corresponding to the first cluster, $\Span(\bm{G}_{j,1})$ by standard PCA on $[\lhat_{\that_j+(K+1)\alpha+1}, \dots , \lhat_{\that_j+ (K+1)\alpha+\alpha}]$, i.e., by computing its top $|\hat{\mathcal{G}}_{j,1}|$ left singular vectors. Since the cluster's condition number is small (bounded by $g^+$), this works. Denote the basis for the estimated subspace by $\hat{\bm{G}}_{j,1}$. To estimate the subspace corresponding to the second cluster, we project the next set of $\alpha$ $\lhatt$'s orthogonal to $\hat{\bm{G}}_{j,1}$, followed by standard PCA to compute the top $|\hat{\mathcal{G}}_{j,2}|$ left singular vectors \cite{rrpcp_perf}. To estimate the $k$-th cluster's subspace, we do a similar thing but with projecting orthogonal to the estimated subspace corresponding to the previous $k-1$ clusters \cite{rrpcp_perf}.
%(the first cluster's estimated subspace)

%For recovering the $k$-th cluster's subspace, we project a new set of $\alpha$ $\lhat_t$'s orthogonal to the estimated subspace corresponding to the previous $k-1$ clusters, followed by PCA on these projected $\lhatt$'s. %$\Span([(P_j)_{\hat{\mathcal{G}}_{j,1}}, (P_j)_{\hat{\mathcal{G}}_{j,2}} \dots,  (P_j)_{\hat{\mathcal{G}}_{j,k-1}}])$, followed by standard PCA.
%By generalizing the analysis approach for p-PCA, it is possible to show that this procedure reduces the subspace error to $r \zeta$.
%
%Cluster PCA is done after the new subspace has been accurately estimated, i.e., after $\that_j+K\alpha$, and hence the error $\et$ in the estimates $\lhatt$ used by cPCA is very small.

%We delete $\Span(\P_{j,\old})$ at $t= \that_{j+1}$ (when the next subspace change is detected). To do this we use the $\lhat_t$'s from $t=\that_{j+1}-2\alpha-(\vartheta_j+1)\alpha$ to $t=\that_{j+1}-2\alpha$. The first $\alpha$ frames are used to detect the clusters automatically and the next $\vartheta \alpha$ frames are used to estimate the eigenvectors of each of the $\vartheta_j$ clusters.
%We do c-PCA every time a new subspace change is detected. At $t=\that_{j+1}$, we use the $\lhat_t$'s from $t=\that_{j+1}-(\vartheta+3)\alpha$ to $t=\that_{j+1}-2\alpha$ for the above. The first $\alpha$ frames are used to detect the clusters automatically and the next $\vartheta \alpha$ frames are used to estimate the eigenvectors of each cluster.




\section{Proof Outline for Theorem \ref{thm1_cor} and Corollary \ref{thm1_cor_corol}} \label{outline}
%
The proof proceeds by induction.
Consider the $j$-the subspace change interval. %Let $\P_{*}:= \P_{t_{j-1}}$, $\P_\new:= \P_{t_j,\new}$ and let $\Phat_*:=\Phat_{t_j-1}$.
Let $\bm{P}_* := \P_{t_{j-1}} = \P_{t_j-1}$, $\P_{\new}:=\P_{t_j,\new}$, and $\Phat_* := \Phat_{\that_{j-1}+K\alpha+(\vartheta+1)\alpha}$.
Assume that there have been no (false) change detects in the interval $[\that_{j-1}+K\alpha+(\vartheta+1)\alpha+1, t_j-1]$. Thus, $\Phat_{t_j-1} = \Phat_*$. Assume also that the subspace, $\Span(\P_{t_j-1})=\Span(\P_{*})$, has been accurately recovered, i.e., $\SE_{t_j-1} = \mathrm{dif}(\Phat_*,\P_*) \le  r \zeta$.
Conditioned on this, we use the following steps to show that, whp, the same conclusions hold at $t=t_{j+1}-1$ as well.
\ben
\item First, we  show that the subspace change is detected within a short delay of $t_j$. We show that $t_j \le \that_j \le t_j + 2 \alpha$ whp. This is done in Lemma \ref{det}.
%In particular, it shows that the change is detected either at $\that_j = u_j \alpha$ or at $\that_j = (u_j+1) \alpha$ where $u_j = \lceil t_j/\alpha \rceil$.

\item At $t=\that_j + \alpha$, the first projection-PCA step is done to get the first estimate, $\Phat_{\new,1}$, of $\Span(\P_{\new})$. This computes the top singular vectors of $[\lhat_{\that_j+1}, \lhat_{\that_j+2}, \dots, \lhat_{\that_j+\alpha}]$ projected orthogonal to $\Span(\Phat_*)$.
In the interval $[t_j, \that_j + \alpha-1]$, the new subspace is not estimated at all, i.e., $\Phat_t = \Phat_*$ while $\P_t = [\P_* \ \P_\new]$ and so $\SE_t \le 1$. Thus, the noise seen by the projected sparse recovery step, $\bm{b}_t$, is the largest in this interval. Hence the error $\et$ is also the largest for the $\lhatt$'s used in the first projection-PCA step. However, due to slow subspace change, even this error is not too large. Because of this, and because $\P_\new$ is dense, %$\et$ is approximately sparse with support $\T_t$ and $\T_t$ follows Model \ref{sbyrho},
 we can argue that $\Phat_{\new,1}$ is a good estimate. We show that $\mathrm{dif}([\Phat_* \ \Phat_{\new,1}], \P_\new) \le 0.19 < 1$.  Thus, at this time, $\SE_t=\mathrm{dif}([\Phat_* \ \Phat_{\new,1}], [\P_* \ \P_\new]) \le r \zeta + 0.19$. This is shown in Lemmas \ref{pPCA} and \ref{zetadecay}.

\item At $t=\that_j + k\alpha$,  for $k=1,2,\dots, K$, the $k$-th projection-PCA step is done to get the $k$-th estimate, $\Phat_{\new,k}$.  This computes the top singular vectors of $[\lhat_{\that_j+(k-1)\alpha+1}, \lhat_{\that_j+(k-1)\alpha+2}, \dots, \lhat_{\that_j+k\alpha}]$ projected orthogonal to $\Span(\Phat_*)$.
%    We show that this estimate has an error less than $0.19\cdot0.1^{k-1} + 0.15 r_\new \zeta$ w.r.t. $\Span(P_{t_j,\new})$. Thus, at this time, $\SE_t \le r \zeta + 0.19\cdot0.1^{k-1} + 0.15 r_\new \zeta$. %The reason for this decrease in error is explained earlier.
    After the first projection-PCA step, $\Phat_t = [\Phat_* \ \Phat_{\new,1}]$ and this reduces $\bm{b}_t$ and hence $\et$ for the $\lhatt$'s in the next $\alpha$ frames. This fact, along with the fact that $\et$ is approximately sparse with support $\T_t$ and $\T_t$ follows Model \ref{sbyrho}, in turn, imply that the perturbation seen by the second projection-PCA step is even smaller. So $\Phat_{\new,2}$ is a more accurate estimate of $\Span(\bm{P}_\new)$ than $\Phat_{\new,1}$. Repeating the same argument, the third estimate is even better and so on. Under the theorem's assumptions, we can show that $\mathrm{dif}([\Phat_* \ \Phat_{\new,k}], \P_\new) \le 0.19\cdot0.1^{k-1} + 0.15 r_\new \zeta$ and so, at $t=\that_j+k \alpha$, $\SE_t \le r \zeta + 0.19\cdot0.1^{k-1} + 0.15 r_\new \zeta$. This is shown in Lemmas \ref{pPCA} and \ref{zetadecay}. The most important idea here is to use the fact that $\et$ is approximately supported on $\T_t$ (shown in Lemma \ref{cslem_cor}) and the support change model on $\T_t$ (this is used in Lemma \ref{blockdiag1}).
    %    Lemma \ref{pPCA} follows by combining Lemma \ref{zetakbnd} with Lemmas \ref{Ak_cor}, \ref{Akperp_cor} and \ref{calHk_cor}.

%    This is repeated $K$ times with $K$ chosen so that $\mathrm{dif}([\Phat_* \ \Phat_{\new,K}],\bm{P}_{\new}) \leq r_{\new}\zeta$.

    %Lemma \ref{pPCA} uses Lemma \ref{cslem_cor} (the projected sparse recovery lemma) to show that the support is exactly recovered and to obtain a closed form expression for $\et$. It then
    % (it happens because a more accurate subspace estimate is used in the projected sparse recovery step for the next set of $\alpha$ frames and this results in a more accurate estimate of $\xt$ and hence of $\lt$ for this period).

\item The above is repeated $K$ times with $K$ set to ensure that, by $t=\that_j + K\alpha$, $\mathrm{dif}([\Phat_* \ \Phat_{\new,K}], \P_\new) \le r_\new \zeta$ and so, at this time, $\SE_t \le (r + r_\new) \zeta$.

\item In the interval $[\that_j + K\alpha+1, \that_j + K\alpha+ (\vartheta+1) \alpha]$, cluster PCA is done to delete $\Span(P_{t_{j}, \old})$. At the end of this step, we can show that the bound on $\SE_t$ has reduces from $(r + r_\new) \zeta$ to $r \zeta$.  This is proved in Lemmas \ref{cluster_lem}, \ref{cPCA} and \ref{zetadecay}.
%The cluster PCA step first involves correct cluster estimation. This is followed by $\vartheta$ steps of cluster PCA.
%    $\mathrm{dif}(\Phat_{t,*},\P_{(j),\ex}) \le (r_{j-1} - r_{j,\old}) \zeta$. We already had $\mathrm{dif}(\Phat_{t,\new}, \P_{(j),\new}) \le r_{j,\new} \zeta$ (from previous step). Thus, at this time, $\SE_t \le  (r_{j-1} - r_{j,\old}) \zeta +  r_{j,\new} \zeta = r_j \zeta < r \zeta$.
%The cluster PCA step first involves correct cluster estimation. Lemma \ref{cluster_lem} proves that this is done correctly whp. This is followed by estimating the subspace corresponding to each cluster accurately. The $k$-th cluster is estimated by projecting a new set of $\alpha$ $\lhatt$'s orthogonal to the previously estimated cluster subspaces followed by PCA. Lemma \ref{cPCA} and item 3 of Lemma \ref{zetadecay} show that this is done accurately whp.

\item Finally, we also argue that there are no (false) subspace change detects for any $t \in [\that_j + K \alpha + (\vartheta+1) \alpha+1, t_{j+1}-1]$. This ensures that $\that_{j+1} \ge t_{j+1}$. This is done in Lemma \ref{falsedet_del}.
\een
To prove the theorem, we first show that the initial subspace is recovered accurately enough, i.e., $\SE_t \le r \zeta$ at $t=t_\train+1$, whp. This is done in Lemma \ref{initsub_cor}. Then, repeating the above argument for each subspace change period, we can obtain the subspace error bounds of the theorem. We set $t_\train$ and $\alpha$ to ensure that the probability of the good events is at least $1-3n^{-10}$. The sparse recovery error bounds can be obtained by using these bounds and quantifying the discussion of Sec. \ref{algo_sec}. This is done in Lemma \ref{cslem_cor}.

The main part of the proof is the analysis of the projection-PCA steps (for subspace addition) and the cluster PCA steps (for subspace deletion). We explain its key ideas next. Assume for this approximate analysis that $\wt=0$ and that $\mathrm{dif}(\Phat_*, \P_*)=0$ (previous subspace is perfectly estimated).
In the $k$-th projection-PCA step the goal is to bound $\zeta_{\new,k}:=\mathrm{dif}([\Phat_*, \Phat_{\new,k}], \P_\new)$ conditioned on ``accurate recovery so far". Here ``accurate recovery so far" means $\mathrm{dif}(\Phat_*, \P_*) \approx 0$ and $\zeta_{\new,k-1} \le \zeta_{\new,k-1}^+$. Before $k=1$, there is no estimate of $\P_\new$ and thus we have $\zeta_{\new,0} \le \zeta_{\new,0}^+=1$.
%where the value of the upper bound $\zeta_{\new,k-1}^+$ will be derived below

We first use the $\sin \theta$ theorem \cite{davis_kahan} (Theorem \ref{sintheta}) to get a bound on $\zeta_{\new,k}$. This is done in  Lemma \ref{zetakbnd}.
We then bound the terms in this bound using the matrix Azuma inequality from \cite{tail_bound} (Corollaries \ref{azuma_hermitian} and \ref{azuma_norm}). This is done in Lemmas \ref{Ak_cor}, \ref{Akperp_cor} and \ref{calHk_cor}.
%The matrix Azuma is significantly harder to apply than matrix Hoeffding used in \cite{rrpcp_icassp15,rrpcp_isit15}. This is because we need to get the sums of conditional expectations of the quantities in each term in a form that their spectral norm can be bounded easily. The obvious way of doing this can lead to very loose bounds. To get the desired bounds, one need to rewrite $\lt$ in terms of past $\bnu_t$'s and use the fact that %$b^\alpha < (r_\new \zeta)$ (is very small) and that $\sum_{\tau=t-\alpha+1}^t b^t \le 1/(1-b) \le 1/(1-b_0) < 1.12$. In words, the contribution of very old $\bnu_t$'s is negligible and the contribution due to the last $\alpha$ $\bnu_t$'s is only slightly larger than that of one $\bnu_t$ (because $b \le b_0=0.1$).
%
%
Using the $\sin \theta$ theorem followed by using matrix Azuma for lower bounding $\lambda_{\min}(\frac{1}{\alpha} \sum_t (I - \Phat_* \Phat_*{}') \lt \lt' (I - \Phat_* \Phat_*{}'))$, we can conclude that
\bea
\zeta_{\new,k} \lesssim  \frac{ \|\mathrm{perturbation}\|_2 }{\frac{1}{1-b^2} \lambda_\new^- - \epsilon - \|\mathrm{perturbation}\|_2 }
\lesssim  \frac{ 2 \big\|\frac{1}{\alpha} \sum_t (I - \Phat_* \Phat_*{}') \lt \et' \big\|_2 +  \big\|\frac{1}{\alpha} \sum_t \et \et'\big\|_2}{ \frac{1}{1-b^2}\lambda_\new^-  - \epsilon - (2\|\frac{1}{\alpha} \sum_t (I - \Phat_* \Phat_*{}') \lt \et' \big\|_2 + 2\big\|\frac{1}{\alpha} \sum_t \et \et'\big\|_2)}
\label{zetanew_approx}
\eea
Here $\mathrm{perturbation} = \frac{1}{\alpha} \sum_t (I - \Phat_* \Phat_*{}') \lhatt \lhatt' (I - \Phat_* \Phat_*{}') - \frac{1}{\alpha} \sum_t (I - \Phat_* \Phat_*{}') \lt \lt' (I - \Phat_* \Phat_*{}')$. Since $\sum_t (\lhatt \lhatt' - \lt \lt') = \sum_t (\lt \et' + \et \lt' + \et \et')$, the bound used in the second inequality above follows.
The next task is to bound the two perturbation terms using the matrix Azuma inequality. This is done in Lemma \ref{calHk_cor}.
As explained in Sec \ref{algo_sec}, under ``accurate recovery so far", it can be shown that $\et$ satisfies \eqref{etdef_0} and that $ \big\|\invterm \big\|_2 \le 1.2$. This is proved in Lemma \ref{cslem_cor}. Notice that, when $\wt=0$, $\et$ is exactly supported on $\T_t$. Using the expression for $\et$, expanding $\lt$ in terms of $\bnu_\tau$'s, manipulating the resulting terms carefully (as explained in Sec \ref{general_decomp}), and applying the matrix Azuma inequality, one can show that, whp,
\[
\big\|\frac{1}{\alpha} \sum_{t=t_0}^{t_0+\alpha-1} (\I - \Phat_* \Phat_*{}') \lt \et' \big\|_2 \le 4 \epsilon + \frac{1}{\alpha}\frac{b^2}{1-b^2} (r\gamma^2) + \mathrm{LargeTerm}_k
\]
where $t_0 = \that_j+(k-1)\alpha+1$ is the first time instant of the $k$-the projection-PCA interval and
\[
\mathrm{LargeTerm}_k:=\big\|\frac{1}{\alpha} \sum_{t=t_0}^{t_0+\alpha-1} \sum_{\tau=t_0}^{t}  b^{2t-2\tau}  \P_\new \Lamtnew \P_\new' (\I - \Phat_* \Phat_*{}' - \Phat_{\new,k-1} \Phat_{\new,k-1}{}') \ITt \invterm \ITt' \big\|_2.
\]
%we use different approaches for $k=1$ and $k > 1$.   (there is no estimate of the new subspace so far)
In the above, $\epsilon$ is very small (comes from applying Azuma for zero-mean terms). The second term is also very small since $1/\alpha \le (r_\new \zeta)^2$. Thus, $\mathrm{LargeTerm}_k$ is the only significant term. To bound it, for $k=1$, we use the fact that $\Phat_{\new,k-1} = \Phat_{\new,0} = [.]$ and hence $(I - \Phat_* \Phat_*{}' - \Phat_{\new,k-1} \Phat_{\new,k-1}{}') \P_\new \approx \P_\new$ and $\P_\new$ is dense. From Model \ref{dense_model}, $ \big\| \P_\new{}' \ITt \big\|_2 \le 0.02$. Thus, using $ \big\|\invterm \big\|_2 \le 1.2$ and slow subspace change, \eqref{anew_small}, we get that, for $k=1$,
\[
\big\|\frac{1}{\alpha} \sum_{t=t_0}^{t_0+\alpha-1} (I - \Phat_* \Phat_*{}') \lt \et' \big\|_2  \lesssim  \big\|\mathrm{LargeTerm}_1 \big\|_2 \le \frac{1}{1-b^2} 1.2 \cdot 0.02 \cdot \lambda_\new^+ \le \frac{1}{1-b^2} 1.2 \cdot 0.02 \cdot 3 \lambda^-  = 0.072 \frac{1}{1-b^2}\lambda^-.
\]

%$\bm\Phi_{k-1}
For $k>1$, we cannot show that $ (\I - \Phat_* \Phat_*{}' - \Phat_{\new,k-1} \Phat_{\new,k-1}{}') \P_\new$ is dense\footnote{The partial result of \cite{rrpcp_perf} assumed that this holds and then used the above approach to get a performance guarantee.}. Thus we use a different approach. We apply the Cauchy-Schwartz inequality (Lemma \ref{CSmat}) with $\bm{X}_t:=\sum_{\tau=t_0}^{t}  b^{2t-2\tau}  \P_\new \Lamtnew \P_\new' (I - \Phat_* \Phat_*{}' - \Phat_{\new,k-1} \Phat_{\new,k-1}{}')$ and $\bm{Y}_t:=\ITt \invterm \ITt'$, followed by using Model \ref{sbyrho} on $\T_t$ to bound  $\lambda_{\max}( \frac{1}{\alpha} \sum_{t=t_0}^{t_0+\alpha-1} \bm{Y}_t \bm{Y}_t')$.

It is easy to see that $\ds \lambda_{\max}( \frac{1}{\alpha} \sum_{t=t_0}^{t_0+\alpha-1} \bm{X}_t \bm{X}_t') \le \max_t \|\bm{X}_t\|_2^2$ and $\ds \|\bm{X}_t\|_2 \le \frac{1}{1-b^2} \lambda_\new^+ \zeta_{\new,k-1}^+ \le  3 \zeta_{\new,k-1}^+  \frac{1}{1-b^2}\lambda^-$. % (using \eqref{anew_small}).

We bound $\ds \lambda_{\max}( \frac{1}{\alpha} \sum_{t=t_0}^{t_0+\alpha-1} \bm{Y}_t \bm{Y}_t')$ by using Model \ref{sbyrho} on support change. This is done in Lemma \ref{blockdiag1}. This lemma exploits the fact that $\ds \frac{1}{\alpha} \sum_t \bm{Y}_t \bm{Y}_t' = \frac{1}{\alpha} \sum_t \ITt (\invterm)^2 \ITt'$ is a block-banded matrix and, for each block, the summation is not over $\alpha$ frames but only over $\beta$ frames with $\beta$ being much smaller. For example, if Model \ref{sbyrho} holds with $\rho=1$, this matrix is block diagonal; if it holds with $\rho=2$, then it is block-tridiagonal and so on. Thus, using $\|\invterm\|_2 \le 1.2$, we can show that $\lambda_{\max}( \frac{1}{\alpha} \sum_{t=t_0}^{t_0+\alpha-1} \bm{Y}_t \bm{Y}_t') \le \frac{1}{\alpha} \rho^2 \beta (1.2)^2 \le 0.0001 \cdot (1.2)^2$.

By Cauchy-Schwartz and the above bounds, we can conclude that, for $k>1$,
\[
\big\|\frac{1}{\alpha} \sum_{t=t_0}^{t_0+\alpha-1} (I - \Phat_* \Phat_*{}') \lt \et' \big\|_2  \lesssim \big\| \mathrm{LargeTerm}_k \big\|_2 \le
 \sqrt{0.0001 \cdot (1.2)^2} \cdot  3 \cdot \zeta_{\new,k-1}^+   \frac{1}{1-b^2}\lambda^- = 0.036\cdot \zeta_{\new,k-1}^+  \frac{1}{1-b^2}  \lambda^-
%
\]
%By manipulating terms followed by application of matrix Azuma, followed by using the support change lemma, Lemma \ref{blockdiag1},

Using an approach similar to the one outlined above one can also bound the $\et \et'$ term. This is actually easier to bound because one does not need Cauchy-Schwartz.
For $k=1$, we get
\[
\big\|\frac{1}{\alpha} \sum_{t=t_0}^{t_0+\alpha-1} \et \et' \big\|_2 \lesssim \rho^2 \beta (1.2)^2 \cdot 0.02^2 \frac{1}{1-b^2} 3 \lambda^- \le 0.0001 \cdot 1.44 \cdot 0.02^2 \cdot 3 \frac{1}{1-b^2}\lambda^- <0.00002 \frac{1}{1-b^2}\lambda^-.
%\sqrt{0.0001 \cdot 1.44} \cdot 3 \cdot 0.83^{k-1}  \frac{1}{1-b^2}  \lambda^-.
\]
%(the above also uses denseness of $\P_\new$)
and for $k>1$,
\[
\big\|\frac{1}{\alpha} \sum_{t=t_0}^{t_0+\alpha-1} \et \et' \big\|_2 \lesssim \rho^2 \beta (1.2)^2 \cdot (\zeta_{\new,k-1}^+ )^2  \frac{1}{1-b^2} 3 \lambda^- \le 0.0001 \cdot 1.44 \cdot 3 \cdot (\zeta_{\new,k-1}^+)^2  \frac{1}{1-b^2}\lambda^- < 0.075 (\zeta_{\new,k-1}^+)^2  \frac{1}{1-b^2}\lambda^-
%\sqrt{0.0001 \cdot 1.44} \cdot 3 \cdot 0.83^{k-1}  \frac{1}{1-b^2}  \lambda^-.
\]

Using the above bounds in \eqref{zetanew_approx} and using $\lambda_\new^- \ge \lambda^-$, we can conclude that,
\[
\zeta_{\new,1}^+ \lesssim 0.19, \ \ \zeta_{\new,k}^+ \lesssim \frac{2 \cdot 0.036 \cdot \zeta_{\new,k-1}^+  +  0.075 (\zeta_{\new,k-1}^+)^2  }{1 - \mathrm{NumeratorTerm}}
%< \frac{0.072 \zeta_{\new,k-1}^+  + 0.075 (\zeta_{\new,k-1}^+)^2  }{1 - \mathrm{NumeratorTerm}}
\]
Here $\mathrm{NumeratorTerm}$ refers to the expression from the numerator. From the above, it is easy to see that $\zeta_{\new,2}^+ \lesssim 0.19$ and, proceeding similarly, $\zeta_{\new,k}^+ \lesssim 0.19$. Using this to get a loose bound on $\mathrm{NumeratorTerm}$, we can conclude that $\zeta_{\new,k}^+ \lesssim 0.1 \zeta_{\new,k-1}^+ \le 0.19 \cdot 0.1^{k-1}$.

The above approximate analysis ignores the fact that $\Span(\Phat_*) \neq \Span(\P_*)$. It also ignores the unstructured noise term $\wt$ and the other small terms that come with each application of matrix Azuma. With incorporating all this, and with using $\mathrm{dif}(\Phat_*,\P_*) \le r \zeta$ (instead of zero), we can conclude that $\zeta_{\new,k} \le \zeta_{\new,k}^+ \le 0.19 \cdot 0.1^{k-1} + 0.15 r_\new \zeta$. By picking $K$ carefully, we get that $\zeta_{\new,K} \le r_\new \zeta$ and thus $\SE_t \le (r+r_\new)\zeta$ after the $K$-the projection PCA step.

The analysis of cluster PCA is a significant generalization of the above ideas. The slow subspace change assumption is replaced by the clustering assumption at various places in its proof.




%
%
%
%In doing the above, the term that is most tricky to bound is the dominant perturbation term for projection-PCA, $\sum_{t = \that_j+(k-1)\alpha+1}^{\that_j+k\alpha} (\I - \Phat_{t-1} \Phat_{t-1}{}') \lt \et'$.
%%The fact that $\et$ is approximately supported on $\T_t$ (see eq??) and the model on $\T_t$ can be used used to get a tight enough bound on this term.
%To be able to apply matrix-Azuma, we need to bound the spectral norm of a matrix that is the sum of certain conditional expectations of matrices obtained after expanding $\lt$ in terms of $\bnu_t$ in the above term.
%By using Cauchy-Schwartz for matrices, its square can be bounded by the spectral norm of a full matrix times the spectral norm of a matrix that is permutation similar to a block-banded matrix. For example, when $\rho=1$, the block-banded matrix will be block-diagonal, when $\rho=2$, it will be block-tridiagonal, and so on. The spectral norm of the full matrix can be shown to be small by using the slow subspace change assumption.
%The spectral norm of a block-banded matrix is proportional to the number of bands times the norm of any one block and this is usually much smaller than if this matrix were dense.
%We get a block-banded matrix in the above proof because $\et$ is approximately supported on $\T_t$ and $\T_t$ follows Model \ref{sbyrho}.



\subsection{Novelty in proof techniques} \label{novelty}
This work has two key contributions - it analyzes ReProCS with the deletion step (done via cluster PCA), and it obtains a complete result for ReProCS and ReProCS-cPCA for the case when the $\lt$'s are correlated over time.

While the overall proof structure described above is similar to that used in \cite{rrpcp_isit15}, the proof approach for proving the ``main lemmas" is quite different for the correlated $\lt$'s case. The first such difference is seen in Fact \ref{ltbnds} which shows how to bound $\|(I - \Phat_{t-1} \Phat_{t-1}{}') \lt\|_2$ for when $\lt$ is correlated over time. This is used to prove Lemma \ref{cslem_cor}.
The second and most significant difference is in proving the matrix-Azuma-based lemmas for projection-PCA and for cluster PCA. These are proved in Sec \ref{3_pfs} and \ref{3_pfs_del}. The matrix Azuma inequality \cite[Theorem 7.1]{tail_bound} is significantly harder to apply than the matrix Hoeffding \cite{tail_bound}. There are two reasons for this. First we need to get the sums of conditional expectations of quantities needed to apply this result in a form that can be bounded easily. The simplest way of doing this can lead to loose bounds. To get the desired bounds, we need to rewrite $\lt$ in terms of past $\bnu_t$'s and use the fact that $b^\alpha < (r_\new \zeta)$ (is very small) and that $\sum_{\tau=t-\alpha+1}^t b^t \le 1/(1-b) \le 1/(1-b_0) < 1.12$. In words, the contribution of very old $\bnu_t$'s is negligible and the contribution due to the last $\alpha$ $\bnu_t$'s is only slightly larger than that of one $\bnu_t$.%

The third main difference is the analysis of the automatic cluster estimation step and of the cluster PCA algorithm for deleting the subspace. The fact that the former is correct whp is shown in Lemma \ref{cluster_lem}. This uses Lemma \ref{cluster_lem_azuma} and the separation condition from Model \ref{clust_model} to show that, whp, the clusters obtained by using a threshold of $\ghatp$ on the condition numbers of the eigenvalues of the empirical covariance matrix computed with the $\lhatt$'s are exactly the same as the true clusters defined in Model \ref{clust_model}. The analysis of cluster PCA (Lemma \ref{cPCA}) relies on matrix-Azuma-based Lemmas \ref{Atil_cor}, \ref{Atilperp_cor}, and \ref{Htil_cor}. These are new too and are proved using a significant generalization of the approach used for analyzing the projection-PCA step.
%Lemmas \ref{Ak_cor}, \ref{Akperp_cor}, and \ref{calHk_cor} that analyze the projection-PCA step.



%\section*{To Do}
%- Lemma \ref{zetadecay} and its proof; propagate the new expressions to rest of the paper, e.g., to value of $K$ / other places / proof outline section (JZ - DO NOT EDIT the first part file - better to email me what needs edited or copy/paste the edits into a new file)
%
%- Bound on $\bb$ - get probabilistic bound.
%
%- add back $\tilde{A}$ etc in deletion proof section.
%
%- Introduction and Notation

